Numerical Computation of Weil-Peterson Geodesics in the Universal Teichm\"uller Space

We propose an optimization algorithm for computing geodesics on the universal Teichm\"uller space T(1) in the Weil-Petersson ($W P$) metric. Another realization for T(1) is the space of planar shapes, modulo translation and scale, and thus our algorithm addresses a fundamental problem in computer vision: compute the distance between two given shapes. The identification of smooth shapes with elements on T(1) allows us to represent a shape as a diffeomorphism on $S^1$. Then given two diffeomorphisms on $S^1$ (i.e., two shapes we want connect with a flow), we formulate a discretized $W P$ energy and the resulting problem is a boundary-value minimization problem. We numerically solve this problem, providing several examples of geodesic flow on the space of shapes, and verifying mathematical properties of T(1). Our algorithm is more general than the application here in the sense that it can be used to compute geodesics on any other Riemannian manifold.

==> content/PL-minimization.tex <==
\section*{Energy minimization algorithms}
We consider here the problem of minimizing the discrete path length given by 
\begin{align}\label{eq:discrete-energy}
  E(v) = \frac{1}{N} \sum_{n=1}^N (v^n)^T H^n v^n.
\end{align}
The vector $v$ contains the Lagrangian velocity field at particle locations
$(\theta^{n m})_{m, n = 1}^{M, N}$, where $n$ denotes time discretization and
$m$ denotes discretization on $S^1$. I.e., the velocity field at location
$\theta^{n m}$ has value $v^{n m}$. We use the column-vector notation $v^n =
(v^{n m})_{m=1}^M$. We assume a forward-Euler time integration scheme so that
$\theta^{n m} = \theta^{1 m} + \frac{1}{N} \sum_{q=1}^{n-1} v^{q m}$. $H^n$ is
the $W P$-minimal metric given by \eqref{eq:wp-minimal-metric} on the particle
locations $\theta^n$. We recall the notation $\widetilde{v^n}$, which represents
the ($W P$-minimal) horizontal lift of $v^n$ onto $\Diff(S^1)$.

\subsection*{A continuous framework}
Consider the following algorithm: relation \eqref{eq:discrete-energy} is
equivalent to 
\begin{align*}
  E(\widetilde{v}) = \frac{1}{N} \sum_{n=1}^N \langle L \widetilde{v^n},
  \widetilde{v^n} \rangle.
\end{align*}
Therefore, the cotangent vector that points in the direction of steepest ascent
at time $n$ is given by 
\begin{align*}
  (\nabla E^\ast)^n = 2 L \widetilde{v^n}.
\end{align*}
In principle then, we seek the elements $w^n$ of $T_h(\Diff(S^1))$ at all times
$n$ that (a) maximize $\sum_n (\nabla E^\ast)^n(w^n)$ and (b) satisfy the
endpoint constraint $\phi_1 - \phi_0 = \frac{1}{N} \sum_{n=1}^N \widetilde{\left(v^n +
w^n\right)}$. However, this constraint is not even satisfied for an initial
guess -- it is only true at the discrete particles. Therefore, it makes sense to
replace the strict continuous constraint with a discretized one at the
particles: $\theta^{(N+1) m} - \theta^{1 m} = \frac{1}{N} \sum_{n=1}^N
\widetilde{\left(v^n + w^n\right)}(\widetilde{\theta}^{n m})$ for all $m = 1, 2,
\ldots, M$, where $\widetilde{\theta^{n m}}$ is the updated particle position
given the perturbed velocity $w^n$: $\widetilde{\theta^{n m}} = \theta^{1 m} +
\frac{1}{N} \sum_{q=1}^{n-1} \widetilde{\left( v^q + w^q
\right)}(\widetilde{\theta^{q m}})$. 
Even with this discretized constraint, we note that the right-hand side of this
constraint does not depend linearly on $w^n$, so without considering a
complicated constrained system, determining an appropriate element in the
tangent space for gradient descent is not easily solvable.

\subsection*{Discrete minimization}
An alternative to the continuous framework is to just consider the discrete
problem and the resulting discrete gradient. We recall expression
\eqref{eq:discrete-energy}, and taking the derivative with respect to $v^{n m}$
yields
\begin{align*}
(\nabla E)^{n m} = \frac{2}{N} (H^n v^n)_m + \frac{1}{N^2} \sum_{q=n+1}^N (v^q)^T
\frac{\partial H^q}{\partial \theta^{q m}} v^q.
\end{align*}
We have used the assumption that forward Euler is used as time-integration
in order to translate $\partial v^{n m}$ into $\partial \theta^{n m}$ and also
to discern that $H^q$ does not depend on $v^{n m}$ for $q \leq n$. Now
\eqref{eq:h-variation} may be used to evaluate the above relation.


==> content/computing-wp-norm.tex <==
We now address computation of the WP norm on tangent vectors to $\Diff(S^{1})$.  Our main task is to compute the $1/2$ and $3/2$ fractional derivatives of a vector field defined on the unit circle.  The following theorem appears in Stein \cite{stein_singular_1970} for the case of $\R^{n}$; we give a proof here of the periodic case in one dimension.

\begin{theorem}
\label{theorem-fractional-derivatives}
Let $f: S^{1} \to \R$ be an $L^{2}$ function.  Then there is a constant $b_{\alpha}$ such that
\begin{align}\label{eq:stein-formula}
\int_{0}^{2\pi} \int_{-\infty}^{\infty} \frac{| f(\theta+s) + f(\theta-s) - 2f(\theta)| ^{2}}{s^{1+2\alpha}} ds d\theta = b_{\alpha} \int_{0}^{2\pi} | f^{(\alpha)}(\theta) |^{2} d\theta
\end{align}
for $0 < \alpha < 2$.
\begin{proof}
By Plancherel,
\begin{align*}
\int_{0}^{2\pi} | f(\theta+s) + f(\theta-s) - 2f(\theta)| ^{2}dx &= 4\sum_{k=-\infty}^{\infty} |\widehat f(k) |^{2} |\cos sk -1 |^{2}
\end{align*}
Hence
\begin{align}
\int_{0}^{2\pi}\int_{-\infty}^{\infty} \frac{| f(\theta+s) + f(\theta-s) - 2f(\theta)| ^{2}}{s^{1+2\alpha}}dsdx &= 4\sum_{k=-\infty}^{\infty} |\widehat f(k) |^{2}\int_{-\infty}^{\infty} \frac{|\cos sk -1 |^{2}}{s^{1+2\alpha}} ds \notag \\
\label{equation-stein-proof-thingy}
&= 4 \sum_{k=-\infty}^{\infty} |\widehat f(k) |^{2} J(k)
\end{align}
where we have set
\begin{align*}
J(k) = \int_{-\infty}^{\infty} \frac{|\cos sk -1 |^{2}}{s^{1+2\alpha}} ds
\end{align*}
Now we observe that $J(k)$ is homogeneous of degree $2\alpha$; indeed, if we replace $k$ by $ck$ for $c \in \mathbb{Z}, c \ne 0$ we have
\begin{align*}
J(ck) &= \int_{-\infty}^{\infty} \frac{|\cos csk -1 |^{2}}{s^{1+2\alpha}} ds \\
&= \int_{-\infty}^{\infty} \frac{|\cos rk -1 |^{2}}{\left(\frac{r}{c}\right)^{1+2\alpha}} \frac{dr}{c} && \text{, setting $r=sc$} \\
&= c^{2\alpha} \int_{-\infty}^{\infty} \frac{|\cos rk -1 |^{2}}{r^{1+2\alpha}} dr \\
&= c^{2\alpha}J(k)
\end{align*}
Therefore \eqref{equation-stein-proof-thingy} is equal to
$4J(1)\sum_{k=-\infty}^{\infty}k^{2\alpha}|\widehat{f}(k)|^{2}$.
Setting $b_{\alpha} = 4 J(1)$ and observing that $J(1)$ converges for $0 < \alpha < 2$ completes the proof.
\end{proof}
\end{theorem}

\mfnote{Perhaps we should keep this as a remark; it seems to clarify.}
\input{content/stein-extension}

\noindent Applying theorem \ref{theorem-fractional-derivatives} to the WP norm, we find the following.
\begin{corollary}
\label{corollary-wp-norm}
\begin{align*}
\| v \|_{WP}^{2} = \frac{\pi}{3} \int_{0}^{2\pi} \int_{-\infty}^{\infty} \left( \frac{4}{s^{4}} - \frac{3}{s^{2}}  \right)| v(\theta+s) + v(\theta-s) - 2v(\theta)| ^{2} ds d\theta 
\end{align*}
\begin{proof}
The constants $b_\alpha$ from Theorem \ref{theorem-fractional-derivatives} take
the values $b_{1/2} = 2\pi$ and $b_{3/2} = \frac{8\pi}{3}$. The equivalence
\eqref{eq:wp-norm-fourier} establishes the result.
\end{proof}
\end{corollary}
%\begin{align*}
%\| v_{t} \|_{\alpha}^{2} &= \int_{\R^{n}} \int_{\R^{n}}  \left( \frac{\partial}{\partial t} \log \| p - q \| \right)^{2} \frac{\ud p \ \ud q}{\|p-q\|^{2\alpha-1}} &&, 0<\alpha<1\\
%\| v_{t} \|_{\alpha}^{2} &= \int_{\R^{n}} \int_{\R^{n}}  \left( \frac{\partial}{\partial t} \log \frac{\| p - q \|}{\| p - \tilde q \|} \right)^{2} \frac{\ud p \ \ud q}{\|p-q\|^{2\alpha-1}} &&, 0<\alpha<2
%\end{align*}

%The WP norm is defined as
%\begin{align*}
%\| v_{t} \|_{WP}^{2} = \sum_{n=2}^{\infty}(n^{3}-n) |a_{n}|^{2}
%\end{align*}
%where $v_{t} = \sum_{-\infty}^{\infty}a_{n}e^{in\theta}$

%We can apply our 1-dimensional versions of Sobolev norms to obtain

%This is our desired expression for computing the fractional derivatives of a vector field on the circle.  It is expressed in terms of distortion of ratios of lengths of intervals about each point.  Logarithms are numerically much more tractable than absolute point locations when points are very near to one another, as is the case in conformal mapping.  In addition, we are able to perform the computation entirely in the spatial domain, without resorting to Fourier transform.  We are actively working on computing geodesic distances using this technique and conjecture that it should be quite robust numerically.


\begin{rem}
Theorem \ref{theorem-fractional-derivatives} also provides an interpretation of the WP norm (or more generally, any Sobolev-type norm on vector fields on the circle) as weighted $L^{2}$ measure of distortion of length ratios, where the weights vary with scale.  Let $v \in \mathrm{vec}(S^{1})$ and let 
\begin{align*}
\phi_{t}(\theta) = \theta + tv(\theta) + o(t)
\end{align*}
Define $I_{t}$ and $J_{t}$ to be the images of intervals of length $s$ about $\theta$ at time $t$:
\begin{align*}
I_{t}(\theta, s) &=  \phi_{t}\left([\theta-s,\theta] \right) \\
J_{t}(\theta, s) &= \phi_{t}\left([\theta, \theta + s] \right)
\end{align*}
Now expand the $L^{2}$ norm of the $\alpha$-th derivative, and at $t=0$ we have
\begin{align*}
\| v^{(\alpha)} \|_{2}^{2} &= \int_{0}^{2\pi} \int_{-\infty}^{\infty} \frac{| v(\theta+s) + v(\theta-s) - 2v(\theta)| ^{2}}{s^{1+2\alpha}} ds d\theta \\
&= \int_{0}^{2\pi} \int_{-\infty}^{\infty}\left| \frac{v(\theta+s) -v(\theta)}{s} - \frac{v(\theta) -  v(\theta-s)}{s} \right| ^{2} \frac{ds}{s^{2\alpha-1}} d\theta \\
&= \int_{0}^{2\pi} \int_{-\infty}^{\infty}\left| \frac{\partial}{\partial t}\log \frac{|I_{t}(\theta, s) |}{|J_{t}(\theta, s)| } \right| ^{2} \frac{ds}{s^{2\alpha-1}} d\theta \\
&= \int_{0}^{2\pi} \int_{-\infty}^{\infty}\left| \frac{\partial}{\partial t} \frac{|I_{t}(\theta, s) |}{|J_{t}(\theta, s)| } \right| ^{2} \frac{ds}{s^{2\alpha-1}} d\theta 
\end{align*}
where the last equality follows since $I_{t}/J_{t} = 1$ at $t=0$.  This converges for $0 < \alpha < 2$.  To obtain similar results for larger $\alpha$, a higher-order finite difference needs to be used, e.g. the third differences can accomodate $0 < \alpha < 3$, as can be seen by repeating the proof of theorem \ref{theorem-fractional-derivatives}.
\end{rem}



==> content/g-matrix-results.tex <==
\section*{The discrete minimal-$W P$ metric}
We explore the properties of the lifting operator and associated metric that
ties a discrete set of values of a velocity field $(v_m)_{m=1}^M$ to an element
$\widetilde{v} \in \Diff(S^1)$. To recall, this lifting operation is defined by
the particle locations $(\theta_m)_{m=1}^M \subset S^1$. Given these locations,
we define the matrix $G$ with entries
\begin{align}\label{eq:g-matrix-entries}
  (G)_{m,n} &= G_f(\theta_m - \theta_n) \\
  \label{eq:greens-function}
  G_f(\theta) &= (1-\cos\theta) \log \left( 2(1-\cos\theta)\right) + \frac{3}{2}
  \cos\theta - 1.
\end{align}
We assume that particles are distinct; then $G$ is a symmetric, positive-definite
matrix, hence invertible. Firstly, we are interested in variations of $G^{-1}$
with respect to particle locations $\theta_m$. The following result allows
simple construction of such variations.
\begin{lemma}\label{lemma:ginv-variation}
  For any $m$, the $M \times M$ matrix $\frac{\partial G^{-1}}{\partial
  \theta_m}$ has rank 2 and is given by
  \begin{align}\label{eq:grad-ginv}
    \frac{\partial G^{-1}}{\partial \theta_m} = G^{-1} V \Lambda V^T G^{-1},
  \end{align}
  where $\Lambda = \mathrm{diag}(\lambda, -\lambda)$, and 
  \begin{align*}
    V &= \frac{1}{\sqrt{2} \|\vec{z}\|} \left[ \vec{z} + \vec{e_m}, -\vec{z} + \vec{e_m}
    \right], \\
    \vec{z} &= \left( G_f'(\theta_n - \theta_m)\right)_{n=1}^N \\
    \lambda &= \| \vec{z} \|,
  \end{align*}
  and $\vec{e_m}$ is the unit vector in entry $m$.
\end{lemma}
\begin{proof}
Formula \eqref{eq:grad-ginv} is a simple application of the parameterized matrix
equality $\frac{\mathd A^{-1}(t)}{\mathd t} = -A^{-1} \frac{\mathd A(t)}{\mathd
t} A^{-1}$. Therefore, we concentrate on obtaining results for $A =
\frac{\partial G}{\partial \theta_m}$. One easily deduces from
\eqref{eq:g-matrix-entries} that $A$ has non-zero entries only in row and column
$m$; indeed row $m$ and column $m$ of $A$ are equal to $\vec{z}$ defined above.
Also, since $G_f$ is an even function, we see that $A$ is symmetric.  Therefore,
we seek to find an eigendecomposition. The structure of $A$ allows one to easily
identify the entire $\R^M$-space orthogonal to $\vec{z}$ and $\vec{e_m}$ as the kernel
of $A$. Then using the eigenvalue equation, one obtains the eigenvalues as $\pm
\|\vec{z}\|$ and the eigenvectors as $\vec{e_m} \pm \vec{z}$.
\end{proof}
We now recall the matrix $H = G^{-1} P$, where $P$ is an orthogonal projector
defined as $P = I - U Q^{-1} U^T G^{-1}$, and $Q = U^T G^{-1} U$. This is the true
lifting matrix: the $W P$-minimal horizontal lift $\widetilde{v}$ is given by 
\begin{align*}
  \widetilde{v} = \sum_{m=1}^M \left(H v\right)_m G_f(\cdot - \theta_m) + \sum_{j=1}^3 \left(
  Q^{-1} U^T G^{-1} v\right) \phi_j,
\end{align*}
where $\phi_j$ is the basis of $\ker(L)$ that defines $U$. We are, in the end,
interested in variations of $H$ with the $\theta_j$. Note that with an easy
method for constructing variations of $G^{-1}$ given in Lemma
\ref{lemma:ginv-variation}, it is quite easy to construct exact variations of
$H$ using e.g. the product rule of differentiation. For completeness, we include
such details below. 

Straightforward manipulation of formulas yields the following relations for
variations in $H$:
\begin{align}\label{eq:h-variation}
  \frac{\partial H}{\partial \theta_m} &= \frac{\partial G^{-1}}{\partial \theta_m} P +
  G^{-1} \frac{\partial P}{\partial \theta_m}, \\\nonumber
  \frac{\partial Q^{-1}}{\partial \theta_m} &= - Q^{-1} \left( \frac{\partial U^T}{
  \partial \theta_m} G^{-1} U + U^T G^{-1} \frac{\partial U}{\partial \theta_m} + U^T
  \frac{\partial G^{-1}}{\partial \theta_m} U\right) Q^{-1}, \\\nonumber
  \frac{\partial P}{\partial \theta_m} &= -\frac{\partial U}{\partial \theta_m}
  Q^{-1} U^T G^{-1} - U \frac{\partial Q^{-1}}{\partial \theta_m} U^T G^{-1} - U Q^{-1}
  \frac{\partial U^T}{\partial \theta_m} G^{-1} - U G^{-1} U^T \frac{\partial
  G^{-1}}{\partial \theta_m}.
\end{align}
The upshot is that the variation in $H$ with respect to $\theta_m$ is
computable, and not too expensive -- it involves computation of variations in
$G^{-1}$, which are known rank-2 matrices, and of variations of $U$ in
$\theta_m$, which is a $N \times 3$ matrix with only one non-zero row. 

\begin{comment}
Consider now the goal of this exercise: we wish to compute the variation of the
discrete path length
\begin{align*}
 E(v) = \frac{1}{N} \sum_{q=1}^N (v^q)^T H^q v^q,
\end{align*}
with respect to $v^{q m}$ for all $q, m$. We have assumed above a Forward-Euler
integration scheme for the particles for simplicity. With this assumption, then
we can write
\begin{align*}
  (\nabla E)^{n m} = \frac{1}{N} \left( 2 (H^n v^n)_m\right) + \frac{1}{N}
  \sum_{q=n+1}^N (v^q)^T \frac{\partial H^q}{\partial \theta_m} v^q.
\end{align*}
This quantity may now be used in a gradient descent or conjugate gradient type
algorithm.
\end{comment}


==> content/gradient-path-length.tex <==
The length of a curve $\phi:[0,1] \times S^{1} \to S^{1}$ in $\Diff(S^{1})$ is 
\begin{align*}
L[\phi] = \int_{0}^{1} \| \dot \phi_{t} \circ \phi_{t}^{-1} \|_{WP} dt
\end{align*}
It is a fact from variational calculus that minimizing length is equivalent to minimizing energy, so given a pair of points $h_{0}, h_{1} \in \Diff(S^{1})$ we find the geodesic by finding the path $\phi$ of minimum energy
\begin{align}\label{eq:energy-definition}
E[\phi] = \int_{0}^{1} \| \dot \phi_{t} \circ \phi_{t}^{-1} \|_{WP}^{2} dt,
\hskip 10pt \phi_0 = h_0, \hskip 10pt \phi_1 = h_1
\end{align}
Since the space is homogeneous, it is sufficient to consider paths from $h_{0}$ to the identity.  Indeed, given any $h_{0}, h_{1}$, we can write $h_{0} = g \circ h_{1}$ and find the shortest path $\phi(\theta, t)$ from $g$ to the identity.  The shortest path from $h_{0}$ to $h_{1}$ is then given by $\phi(h_{1}(\theta), t)$.  Therefore we consider only paths ending at the identity.

(Careful here... maybe work this next section after discretization into landmark points, where this is finite-dimensional and obvious.  I don't understand implicit ftn thm in more general settings.)  Let $P_{h_{0}}$ be the manifold of all paths in $\phi: S^{1} \times [0,1] \to S^{1}$ which join $h_{0}$ to the identity; this is a submanifold of the manifold of all paths in $\Homeo(S^{1})$.   We construct this as an implicit submanifold given by the constraints that for each $\theta$ we must have
\begin{align}
\label{condition-submanifold-gets-there}
\int_{0}^{1} v_{t}(\phi_{t}(\theta)) dt = h_{0}^{-1}(\theta) - \theta
\end{align}
along with topological constraints, say $\phi_{t}' > 0$ for all $t$.  
\mfnote{I was thinking of the $\theta$'s as particles which initially lie in the range of $h_{0}$, which I think is consistent with how the code was working.}
We now discretize time into $N$ steps and choose $M$ initial particles $\theta_{j}$ in the range of $h_{0}$.  Rather than storing their positions at each time step, we store their velocities $v_{j}(k)$ for $k \in 1,2,3,...,N$.  For each particle $\theta_{j}$, the condition \eqref{condition-submanifold-gets-there} on the velocity field becomes
\begin{align*}
F_{j}(v) = \sum_{k=1}^{N} v_{j}(k) = h_{0}^{-1}(\theta_{j}) - \theta_{j}
\end{align*}
if we use a simple first-order approximation $\phi_{n}(\theta_{j}) = \theta_{j}(0) + \sum_{k=1}^{n}v_{j}(k)$ to compute particle positions at each timestep.  Now let $F$ be the vector-valued function
\begin{align}\label{eq:velocity-constraints}
F(v) = \myvec{F_{1}(v) \\ F_{2}(v)\\ \vdots \\ F_{M}(v)}
\end{align}
\mfnote{Yes, it'll follow from basic ODE results applied to the geodesic equation.  I don't know the exact degree of regularity in $t$ here, but every result I've seen on this question just used the usual trick to convert the geodesic equation to a system of first-order ODEs and then cites the usual stuff.}
In coordinate $v$, where $v(\cdot,t)$ is a vector field on $S^{1}$ for any fixed $t$,  the manifold $P_{h_{0}}$ has tangent space given by $\mathrm{null}[DF]$.  We can compute the path of least energy by finding the constrained gradient of energy $\widetilde \nabla E$; that is, the direction in $T_{\phi}P_{h_{0}}$ in which arc length increases most rapidly.  This is simply the projection onto $T_{\phi}P_{h_{0}}$ of the gradient of arc length in the whole space (i.e. the space of all paths regardless of endpoints).  This is trivial to compute; we will need an easy lemma first for computing the gradient of a function on a submanifold $M$ of a manifold $N$ equipped with an inner product.  Given a function $f:N \to \R$, let $Df$ be its differential.  The next lemma relates the gradient $D(\left.f\right|_{M})$, i.e. the differential of the restriction of $f$ to $M$, to the differential $Df$.
\begin{lemma}\label{lemma:v-projection}
Let $M$ be a smooth submanifold of $N$ with $f: N \to \R$.  Then the vector $v^{*} \in T_{p}M$ given by
\begin{align*}
v^{*} \equiv \mathrm{proj}_{T_{p}M} \left( \nabla f(p) \right)
\end{align*}
maximizes $ \| D ( \left. f\right|_{M})(v) \|$ over all $v \in T_{p}M$.
\begin{proof}
At any point $p$ we may write 
\begin{align*}
\nabla f = (\nabla f)^{T} + (\nabla f)^{\perp}
\end{align*}
where $(\nabla f)^{T}$ and $(\nabla f)^{\perp}$ lie in and orthogonal to $T_{p}M$, respectively.  Then we seek a direction $v^{*} \in T_{p}M$ which maximizes
\begin{align*}
\langle \nabla f, v \rangle = \langle (\nabla f)^{T}, v  \rangle 
\end{align*}
By the Schwarz inequality, this is clearly given by $v^{*} =  (\nabla f)^{T} = \mathrm{proj}_{T_{p}M} \left( \nabla f \right)$.
\end{proof}
\end{lemma}
\noindent In light of the preceding lemma, the gradient is as follows.
\begin{proposition}[Gradient of length]\label{prop:gradient-length}
The gradient of arclength for the fixed-endpoint problem satisfies
\begin{align}\label{eq:gradient-length}
\widetilde \nabla E(v) = \mathrm{proj}_{\mathrm{null} [DF]} \nabla E(v)
\end{align}
where
\begin{align*}
\nabla E(v)(t, \theta) = \frac{2\pi}{3} \int_{-\infty}^{\infty} \left( \frac{4}{s^{4}} - \frac{3}{s^{2}}  \right) \left( v_{t}(\theta+2s) -4 v_{t}(\theta+s) +6v_{t}(\theta) - 4v_{t}(\theta-s) + v_{t}(\theta-2s)\right) ds  
\end{align*}
\begin{proof}
It is sufficient to work at a single timestep.  Let $w \in \Vec(S^{1})$ and write
\begin{align*}
v_{\epsilon} &= v + \epsilon w, \\
D_2[f](\theta;s) &= f(\theta-s) + f(\theta+s) - 2 f(\theta),  \\
D_4[f](\theta;s) &= f(\theta-2 s) - 4 f(\theta - s) + 6 f(\theta) + 4 f(\theta+s)
+ f(\theta + 2 s), \\
\kappa(s) &= \frac{\pi}{3}\left(\frac{4}{s^4} - \frac{3}{s^2}\right).
\end{align*}
Now take the first variation of the squared norm using Corollary \ref{corollary-wp-norm}:
\begin{align*}
\left.\ppx{\epsilon} \right|_{\epsilon=0} \left\| v_{\epsilon} \right\|_{WP}^2 &= 
      2 \int_0^{2 \pi} \int_{-\infty}^\infty \kappa(s) D_2[v](\theta;s) D_2[w](\theta;s)
      \,\dx{s}\,\dx{\theta} \\
  &= 2 \int_{-\infty}^\infty \left\langle \kappa(s)
      D_2[v](\theta;s) \dx{s},\; w(\theta-s) + w(\theta+s) - 2
      w(\theta) \right\rangle \dx{s} \\
  &= 2 \int_{-\infty}^\infty \left\langle \kappa(s) 
      \left( D_2[v](\theta-s; s) + D_2[v](\theta+s; s) - 2 D_2[v](\theta; s) \right), 
      w(\theta) \right\rangle \dx{s} \\
  &= 2 \int_{-\infty}^\infty \left\langle \kappa(s) D_4[v](\theta; s), w(\theta)
  \right\rangle \dx{s}
%\left.\frac{\partial}{\partial \epsilon}\right|_{\epsilon=0} \| v_{\epsilon} \|_{WP}^{2} &= \left.\frac{\partial}{\partial \epsilon}\right|_{\epsilon=0} a \int_{0}^{2\pi} \int_{-\infty}^{\infty} \left( \frac{1}{s^{4}} - \frac{b}{s^{2}}  \right)| v(\theta+s) + v(\theta-s) - 2v(\theta)| ^{2} ds d\theta \\
%&=  a \int_{0}^{2\pi} \int_{-\infty}^{\infty} \left( \frac{1}{s^{4}} - \frac{b}{s^{2}}  \right) \left( v(\theta+s) + v(\theta-s) - 2v(\theta)\right) \left( w(\theta+s) + w(\theta-s) - 2w(\theta)   \right) ds d\theta \\
%&= a \int_{-\infty}^{\infty} \left( \frac{1}{s^{4}} - \frac{b}{s^{2}}  \right) \left( v(\theta+2s) -4 v(\theta+s) +6v(\theta) - 4v(\theta-s) + v(\theta-2s)\right) w(\theta)ds  
\end{align*}
\end{proof}
\end{proposition}
\begin{rem}
Blah blah Fubini? If the operator $D^{(k)}$ denotes the central-difference operator blah blah
\begin{align*}
\langle D^{(k)}f , g \rangle = \langle f, D^{(k)} g \rangle
\end{align*}
in particular, one may interpret the norm obtained by polarization
\begin{align*}
\| f \| = \langle D^{(k)}f, D^{(k)}f \rangle
\end{align*}
etc.  So get inner product etc.
\end{rem}
%\begin{align*}
%\langle D^{(k)}f, D^{(k)}g \rangle = \langle D^{(2k)}f, g \rangle
%\end{align*}
%I.e. if you change variables in the integral, like the proof of the first variation above in proposition 1, you end up with taking more differences on the first function.  It works formally exactly like integration by parts; it's just a discrete analog.  
% The other neat thing is that you can pull the $g$ out of the integral $ds$ and so you can integrate up all the $2k$-th differences first.  This leads to formulas for the differential operator and reproducing kernel expressed entirely in terms of the $2k$-th differences.  Of course they're just the usual powers of the Laplacian and the Riesz/Bessel/whatever kernels, but the formulas are more geometric.}


==> content/la.tex <==
\section{Computations}\label{sec:computations}
In this section we establish the connection computations of the $W P$ norm and
related quantities to some established linear algebra problems. Given an $M
\times N$ matrix $A$, $A^+$ denotes its Moore-Penrose pseudoinverse. For any
$\V{b} \in \R^N$, the vector $A^+ \V{b}$ is the minimum-norm, least squares
solution to $A \V{x} = \V{b}$.  Here, both {\em minimum-norm} and {\em least
squares} refer to the $\ell^2$ (Euclidean) metric on $\V{x}$ and $\V{b}$,
respectively. 

%Suppose we wish to generalize `least squares' to any valid semimetric, say some
%semidefinite quadratic form represented by the square, symmetric, positive
%semidefinte matrix $B$ on $\R^N$. Nothing much changes: this minimum-norm
%(Euclidean) and least squares ($B$) solution to $A \V{x} = \V{b}$ is given by
%$A^+ M \V{b}$, where $M$ is any matrix square root of $B$. I.e. $B = B_R^T B_R$.
%$M$ need not be square.
%
%If we now wish to allow a semimetric on $\R^M$ defined by the semidefinite
%quadratic form $X$, things become a bit more complicated. Let $L$ be any matrix
%square root of $X$: $X = X_R^T X_R$. When $X$ and $B$ are both strictly positive
%definite, a unique solution exists and is given by Van Loan (cite) via a type of
%generalized singular value decomposition. If we allow semidefiniteness in both
%$X_R$ and $B_R$ then uniqueness may violated. Nevertheless, if a unique solution
%exists, a result due to Elden (cite) provides the following minimum-norm, least
%squares solution via a weighted pseudoinverse: let the matrix pair $(A, X_R)$
%admit the following generalized singular value decomposition:
%\begin{align}\label{eq:gsvd}
%  A &= U C P^{-1} \\
%  X_R &= V S P^{-1},
%\end{align}
%where $U$ and $V$ are unitary, $C$ and $S$ are positive diagonal with $C^T C +
%S^T S = I$, and $P$ is invertible. Then if $A \V{x} = \V{b}$ has a unique
%minimum-norm ($X$), least squares ($B$) solution, it is given by $P C^+ U^H M
%\V{b}$. 

\subsection{The WP norm}
In order to compute the horizontal lift $\widetilde{v}$, there is an alternative
to direct computation of the matrix $H$ as defined in Section
\ref{sec:lifting-v}. Here we develop the ideas for a general subspace
$\widetilde{V}_N$ from Section \ref{sec:other-subspaces} and then specialize to
the minimal-norm lift over all $V$. Recalling the goal of interpolating data
$\V{v} \in \R^M$ on $\delta(\mathcal{L}^M)$ with an element from
$\widetilde{V}_N \oplus \ker_V L$, we are essentially trying to find the
minimal norm solution to
\begin{align}\label{eq:full-minnorm-system}
  \left[\begin{array}{cc} \lambda(\Phi) & B \end{array}\right] \left(
  \begin{array}{c} \V{c} \\ \V{w} \end{array} \right) =:
  A \V{x} = 
  \V{v},
\end{align}
where the norm over the coefficients $\V{c}$ is given by the positive (Gram)
matrix $\Phi$ and that over the kernel coefficients $\V{w}$ is zero. Again we
assume that $\widetilde{V}_N$ is total for interpolation on $\mathcal{L}^M$,
implying that $A \V{x} = \V{v}$ has at least one solution. Let $\Phi_0$ be a
block diagonal matrix with $\Phi$ in the upper-left block and a $3 \times 3$
zero matrix in the lower-right block.  Owing to Lemma
\ref{lemma:kernel-totality}, the kernel of $B$ is trivial so long as $M \geq 3$.
Therefore, $\ker(\Phi_0) \cap \ker(A) = \{\V{0}\}$ and a result due to Elden
(cite) ensures that the minimum norm solution to \eqref{eq:full-minnorm-system}
is unique.

Restating \eqref{eq:full-minnorm-system}, we are trying to solve the
minimization problem:
\begin{align}\label{eq:lse-problem}
  \text{minimize} \hspace{0.5cm} \left\| \Phi_0^{1/2} \V{x} \right\|_2
  \hspace{0.5cm} \text{subject to} \hspace{0.5cm}
  A \V{x} = \V{v},
  %\left[\begin{array}{cc} \lambda(\Phi) & B \end{array}\right] \V{x} = \V{v},
\end{align}
where $\Phi_0^{1/2}$ is any matrix square root of $\Phi_0$. (I.e.
$(\Phi_0^{1/2})^T \Phi_0^{1/2} = \Phi_0$.) One of the standard tools for solving
least squares equality constrained problems is the generalized singular value
decomposition (GSVD) (cite). Since $A$ and $\Phi_0$ have the same number of
columns, the GSVD matrix decomposition of $(A, \Phi_0^{1/2})$ is given by 
\begin{subequations}
\label{eq:gsvd}
\begin{align}
  A &= U C X^{-1} \\
  \Phi_0^{1/2} &= V S X^{-1},
\end{align}
\end{subequations}
where $U$ and $V$ are orthogonal matrices, $X$ is invertible, and $C$ and $S$
each have only one non-vanishing diagonal with non-negative entries and satisfy
$C^T C + S^T S = I$. The solution to \eqref{eq:lse-problem} is given by
\begin{align}\label{eq:gsvd-solution}
  \V{x} = \left(\begin{array}{c} \V{c} \\ \V{w}\end{array}\right) &= X C^+ U^T \V{v},
\end{align}
The above matrix mapping $\V{v}$ to $\V{x}$ is a weighted pseudoinverse of $A$
with respect to $\Phi_0^{1/2}$.  The momenta are $\V{m} = U C^{+T} X^T \Phi_0 X
C^+ U^T \V{v}$.  This is a much more stable way to compute momenta than the
explicit matrix relations given in Section \ref{sec:other-subspaces}. The matrix
$X$ is usually very well-conditioned; $U$ is unitary; $C^+$ is a matrix with
only one diagonal of non-zeros and therefore applications of $C^{+}$ can be
accomplished with a simple vector-vector multiply. The norm is
$\|\V{v}\|_{\widetilde{W P},\widetilde{V}_N} = \V{c}^T \Phi \V{c} = \V{v}^T \V{m}$ and naturally
$\V{m} = Q^{-1} P_Q^B \V{v}$ to match \eqref{eq:other-subspace-norm}. 

For the horizontal lift from the whole space $V$, we need only take the space
$\widetilde{V}_N$ to be the $M$-dimensional space of Green's functions centered
at the $\theta_m$. Notable simplifications in this case are that (a) $\Phi = G$,
with $G$ being the Green's function matrix and (b) the momentum and basis
coefficients coincide: $\V{m} = \V{c}$.

We recall that in the case of our discretization in time, the matrix $\Phi_0$
should be replaced by $h^t \Phi_0$ so that the momenta $\V{m}^t$ are scaled
properly.

\subsection{The gradient of the WP norm}
At some time $s^t$, we have seen that if $H = Q^{-1} P_Q^B$, then
$\|\V{v}^t\|_{\widetilde{W P},\widetilde{V}_N} = \V{v}^t H \V{v}^t$. The formula
\eqref{eq:pathlength-discretization} is the objective, and we must compute
variations of this with respect to velocity evaluations. Since the particle
positions are influenced by \eqref{eq:particle-update}, the matrices $H$ and
therefore the path length change in nontrivial ways when we vary $\V{v}^t$. To
simplify the procedure, we fix $t$ and consider only variations in
$\|\V{v}^t\|_{\widetilde{W P}}$ with respect to $\V{v}^r$ for $r = 1,\ldots,T$.

The update \eqref{eq:explicit-particle-update} shows that
$\V{q}^t$ does not depend on $\V{v}^t$. Therefore, $Q^{-1} P_Q^B$ is independent
of $\V{v}^t$. As such, 
\begin{align}\label{eq:wpnorm-variation-velocity}
  \ppx{\V{v}^t} \|\V{v}^t\|^2_{\widetilde{W P},\widetilde{V}_N} = 2 (\V{v}^t)^T Q^{-1} P_Q^B = 2
  (\V{m}^t)^T,
\end{align}
and for any particle $m = 1, 2, \ldots, M$ we have 
\begin{align*}
  \ppx{q^t_m} \|\V{v}^t\|^2_{\widetilde{W P},\widetilde{V}_N} = (\V{v}^t)^T
  \ppx{q^t_m}\left(Q^{-1} P_Q^B\right)
  \V{v}^t,
\end{align*}
where $Q$ and $P_Q^B$ are generated from $\V{q}^t$. Using simple properties of
matrix algebra, a straightforward but messy computation yields a formula for the
variation of the objective with respect to the particle positions.
\begin{lemma}\label{lemma:wpnorm-particle-variation}
Let $\lambda(\Phi')$ be the $M \times N$ matrix with entries
$\lambda(\Phi')_{m,n} = \phi_n'(\theta_m)$ and $B'$ be the $M \times 3$ matrix
with entries $B'_{m,j} = b_j'(\theta_m)$.  For two matrices $C$ and $D$ of the
same size, $C \circ D$ denotes the Hadamard (elementwise) product.  Then 
\begin{align}\label{eq:wpnorm-variation-particle}
 \ppx{\V{q}^t} \|\V{v}^t\|^2_{\widetilde{W P},\widetilde{V}_N} = -2 \left[ \V{m}^t \circ
 \left(\lambda(\Phi') \Phi^{-1} \lambda(\Phi)^T \V{m}^t + B'
 \V{w}^t\right)\right]^T.
\end{align}
In particular, if $\Phi = \delta(\mathcal{L}^M)$, then 
\begin{align}\label{eq:wpnorm-variation-particle-hlift}
 \ppx{\V{q}^t} \|\V{v}^t\|^2_{\widetilde{W P}} = -2 \left[ \V{m}^t \circ
 \widetilde{v}'(\V{q}^t)\right]^T,
\end{align}
where $\widetilde{v}'$ is the derivative of the horizontal lift from $V$.
\end{lemma}
The salient result of Lemma \ref{lemma:wpnorm-particle-variation} is that
computing variations of the $W P$ norm with respect to particles is quite easy
once we have the momentum coefficients $\V{m}$ and kernel coefficients $\V{w}$
in hand from the GSVD. The only difficulty could come in either inverting the
Gram matrix $\Phi$ or in computing entries for $\lambda(\Phi')$. In all the
straightforward choices for $\Phi$ we make, neither is difficult. We can now use
the chain rule to compute the variation of the full objective with respect to
the data $\V{v}$.

\subsection{The gradient of pathlength}
With the gradient of the $W P$ norm computed, computing the pathlength is now
straightforward. Combining \eqref{eq:particle-update},
\eqref{eq:wpnorm-variation-velocity}, and \eqref{eq:wpnorm-variation-particle},
we have
\begin{align*}
  \pfpx{L}{\V{v}^t} = 2 (\V{m}^t)^T - 
                     \sum_{r \neq t} h_r c_{t,r} \pfpx{\|\V{v}^r\|^2_{\widetilde{W
                     P}}}{\V{q}^r},
\end{align*}
where $c_{t,r}$ is given by \eqref{eq:crt-def} and again we recall that the
momenta coefficients already have the scaling factor $h^t$ included.

Although the above equation is an exact formula for the gradient, updating
velocity fields with these values will not respect the endpoint constraint
$\V{q}^1 = \V{q}^0 + \sum_t h_t \V{v}^t$. We therefore project the computed
gradient into the space of admissible updates. Let $\V{h}$ be the $T \times 1$
vector with entries $h_t$; then $P_h = I - \frac{\V{h}\V{h}^T}{\V{h}^T \V{h}}$
is the (Euclidean) orthoogonal projection onto $\ker(\V{h}^T)$. I.e., let $D$ be
the $M \times T$ matrix containing evaluations $D_{m,t} = \ppx{v^t_m} L$. The
update matrix
\begin{align*}
  \widetilde{D} = D P_h
\end{align*}
has rows that lie in $\ker(\V{h}^T)$, which will respect the endpoint
conditions. We can then perform a gradient update step via
\begin{align*}
  V \gets V + \varepsilon \widetilde{D}
\end{align*}
for some small $\varepsilon$.

\subsection{Simultaneous minimization}
Before explicitly defining the algorithm, we explore one more relevant topic.
The solution defined by e.g. \eqref{eq:gsvd-solution} defines the lift at one
point in time by subtracting out kernel elements that minimize the norm at the
{\em same} moment in time. Our algorithm will be computing such kernel elements
at each point in time, and there is no explicit coupling of the kernel
coefficients. The result is that the kernel coefficients do not vary smoothly in
time. 

Mathematically there is nothing wrong with this, but our experience shows that
implementing this minimization technique introduces spurious numerical artifacts
since we have a discrete-time integration method that works best with smooth
evolutions. Since our initial and final fingerprints are fixed, there is a
kernel element constant in time that changes the chart of $\phi_0$ to that of
$\phi_1$. To ameliorate the observed artifacts when we allow the kernel element
to evolve in time, we perform the minimization over all time by picking out a
single collection of kernel coefficients for all points in time. Most of the
formulation remains unchanged, but we present a few details here for
completeness.

Since the interpolation conditions $\lambda$ and the subspace $\widetilde{V}_N$
may change at each point in time, some extra indexing must be introduced.
Let $\lambda^t(\Phi^t)$ denote the $\widetilde{V}_N$ interpolation matrix at time
$s^t$ derived from particle locations $\V{q}^t$, and let $B^t$ denote the kernel
interpolation matrix at $s^t$. $\lambda^t (\Phi^{t\prime})$ and $(B')^t$ are defined as
usual.  Now define the matrices
\begin{align*}
  A &= \left(\begin{array}{cccccc} 
         \lambda^1(\Phi^1) & 0 & 0 & \cdots & & B^1 \\
         0 & \lambda^2(\Phi^2) & 0 & \cdots & & B^2 \\
         0 & 0 & \lambda^3(\Phi^3) & & & B^3 \\
         \vdots & \vdots & & \ddots & & \vdots \\
         & & & & \lambda^T(\Phi^T) & B^T
       \end{array}\right),  \\
  \Phi_0 &= \left(\begin{array}{cccccc} 
          \sqrt{h^1 \Phi^1} & 0 & 0 & \cdots & & 0_{N \times 3}\\
          0 & \sqrt{h^2 \Phi^2} & 0 & \cdots &  & 0_{N \times 3}\\
          0 & 0 & \sqrt{h^3 \Phi^3} & & & 0_{N \times 3} \\
          \vdots & \vdots & & \ddots & & \vdots\\
          & & & & \sqrt{h^T \Phi^3} & 0_{N\times 3}
       \end{array}\right).
\end{align*}
Our solution vector is then given by \eqref{eq:gsvd-solution}, where $\V{m}$ is
of size $N T$ and $\V{w}$ is of size 3. Therefore, the kernel coefficients
$\V{w}$ correspond to the amount of the kernel that is subtracted out for every
point in time. One should be careful to realize that although this allows us to
define momentum coefficients at all points in time, the usual formula $(\V{m}^t)^T
\V{v}^t$ no longer represents the $W P$ norm at time $s^t$: instead the relevant
quantity is
\begin{align*}
  \|\V{v}^t\|^2_{\widetilde{W P}} = (\V{m}^t)^T \left( \V{v}^t - B^t \V{w}\right).
\end{align*}
Of course if we sum over all time, then $\sum_t \| \V{v}^t
\|^2_{\widetilde{V}_N} = \sum_t (\V{v}^t)^T \V{m}^t$.
Using the momenta $\V{m}$, then as before one can show that 
\eqref{eq:wpnorm-variation-particle} holds, where the appropriate superscripts
$t$ must be added.
%\begin{align}\label{eq:wpnorm-ensemble-variation-particle}
% \ppx{\V{q}^t} \left(\sum_{t=1}^T \|\V{v}^t\|^2_{\widetilde{W P}}\right) = -2 \left\{ (\V{m}^t)^T \circ
% \left[(G')^t \V{m}^t + (B')^t \V{w}\right]^T\right\},
%\end{align}
%\aknote{Actually, I'm not sure I know how to prove this, but I know it's true.}
%where $\V{m}^t$ corresponds to the $N$ momenta coefficients at time $s^t$ from
%$\V{m}$.


==> content/minimal-wp-extension.tex <==




==> content/multiple-charts.tex <==
\section{Working in multiple charts}

To address the ``crowding'' problem, we break up the computation of the WP norm into several integrals done in multiple coordinate charts.  This is not too difficult due to invariance of the WP norm under the adjoint action.  The adjoint mapping is the map of the Lie algebra $\mathfrak{g} = T_{e}G$ to itself induced by conjugation $g \mapsto h^{-1} \circ g \circ h$.  That is, for fixed $h$, $Ad_{h}: \mathfrak{g} \to \mathfrak{g}$ is the linearization of conjugation at the identity.  Explicitly, for $v \in \mathfrak{g}$ and $h \in G$, we have
\begin{align*}
Ad_{h}(v) = \frac{v \circ h}{h'}
\end{align*}
An essential property of the WP metric is that for $\phi \in PSL_{2}(\R)$ we have
\begin{align*}
\| Ad_{\phi}v \|_{WP} = \| v \|_{WP}
\end{align*}
(Up to here, this is true.  Now bring the funk...)
%Intuitively, consider the sequence of group elements 
%\begin{align*}
%\phi_{1}^{-1} \circ ... \circ \phi_{n}^{-1} \circ \nu \circ \phi_{m} \circ ... \circ \phi_{1}
%\end{align*}
%which is a sort of discretization of $Ad_{\phi} v$ when $\nu(\theta) = \theta + \epsilon v(\theta)$ and the $\phi_{i}$ are approximately maps of the form $\phi_{i}(\theta) = \theta + \epsilon w_{i}(\theta)$ for $w_{i} \in psl_{2}(\R)$.  Clearly the WP norm of the path will be equal to the length of the path given by $\nu$ alone.
This allows us to rewrite the WP norm as a sum of integrals in different coordinate charts.  Let $I_{j}$, $j=1,2,3,...,K$ be a collection of disjoint open intervals whose closures cover $S^{1}$.  Then write
\begin{align*}
\widetilde v_{j}(\theta) = \sum_{j=1}^{K} \chi_{I_{j}}(\theta)v(\theta)
\end{align*}
Then for any collection of maps $\{ \phi_{j} \}_{j=1}^{K} \subset PSL_{2}(\R)$ we can compute
\begin{align*}
\| v \|_{WP} &= \sum_{j=1}^{K} \| \widetilde v_{j}  \|_{WP} \\
&= \sum_{j=1}^{K} \| Ad_{\phi_{j}} \widetilde v_{j} \|_{WP}
\end{align*}
This makes no sense, yet how could this possibly be false?  (Argue with the floor).


==> content/new-wp-computations.tex <==
\section{Norms and lengths}
In this section we present explicit formulae for lengths of paths.  First we
consider the problem of computing the norm of a vector field on $S^1$, which has
a simple connection to numerical linear algebra. This allows us to compute
lengths of paths. The next section will computational considerations and will
consider computation of the gradient of path length that drives the optimization
algorithm to find geodesics.

\subsection{Lifting the velocity field}\label{sec:lifting-v}
Consider the space of all vector fields on $S^1$, and a subspace on which
$\|\cdot\|_{W P}$ is a proper norm:
\begin{align*}
  V &= \{v: \|v \|_{W P} < \infty\}, & \tilde{V} = \{v \in V: v \perp 
  \ker_V L\}.
\end{align*}
The following material appears for the case of $\R^{n}$ in [CITE Mumford]; we repeat it
here in the case of $S^{1}$ in order to be self-contained.  Let
$\mathcal{L}^{M}$ be the space of configurations of $M$ points $\theta_{1} <
\theta_{2} < ... < \theta_{M}$ on the unit circle and write $\Theta = \left\{
\theta_{1}, \theta_{2}, ..., \theta_{M}  \right\}$. The tangent space
$T_{\Theta}\lm$ is the $M$-dimensional space of vector fields $v = (v_{1},
v_{2}, ..., v_{M})$ supported on the set $\Theta$.  We consider all possible
extensions of $v$ to vector fields defined on the entire circle, and induce a
metric on $\lm$ by defining the norm
\begin{align}\label{eq:v-global-minimizer}
\| v \|_{\widetilde{WP}} \equiv \inf \left\{ \| \widetilde v \|_{WP} : \widetilde{v}(\theta_{j}) = v_{j}  \right\}
\end{align}
Having chosen some basepoint $\Theta$, the tangent space $T_{h}\Diff(S^{1})$
then splits as the direct sum
\begin{align*}
T_{h}\Diff(S^{1}) = T_{h}\Diff(S^{1})_{hor} \oplus T_{h}\Diff(S^{1})_{ver}
\end{align*}
The vertical subspace is the subspace consisting of vector fields which vanish
at all the $\theta_{j}$.  The horizontal subspace is the $M$-dimensional
orthogonal complement of the vertical subspace and hence contains the
norm-minimizing extensions of vectors in $T_{\Theta}\lm$, known as the
\textit{horizontal lifts}.

Working in coordinate $v$ on $P_{h_{0}}$, we may obtain an expression for the
gradient of arc length by considering Green's function for the WP differential
operator $L = -\mathcal{H}(\partial^{3} - \partial)$ ($\mathcal{H}$ is the Hilbert
transform).  This Green's function is known explicitly, see
\cite{kushnarev_teichons_2009}:

\begin{align*}
G(\theta) = 2 \sum_{n=2}^{\infty} \frac{\cos(n\theta)}{(n^{3}-n)} = (1-\cos \theta) \log\left[ 2(1-\cos \theta)  \right] + \frac{3}{2}\cos \theta -1
\end{align*}

\begin{proposition}\label{prop:vector-field-basis}
The set of vector fields
\begin{align*}
\left\{ G(\theta, \theta_{j}) \frac{\partial}{\partial\theta} \right\}_{j=1}^{M}
\end{align*}
is a basis for $T_{h}\Diff(S^{1})_{hor} \cap \widetilde{V}$, the component of the
horizontal subspace on $\widetilde{V}$.
\begin{proof}
By the reproducing kernel property of Green's function, we know that 
\begin{align*}
\langle v, G(\cdot - \theta_{j}) \rangle_{WP} = v(\theta_{j})
\end{align*}
for all $j = 1,2,...,M$ and any vector $v \in T_{h}\Diff(S^{1}) \cap \widetilde{V}$.
In particular, if $v$ is vertical we have
\begin{align*}
\langle v, G(\cdot - \theta_{j} )\rangle_{WP} = v(\theta_{j}) = 0
\end{align*}
so $G\frac{\partial}{\partial\theta}$ is orthogonal to the vertical subspace;
i.e. $v \in T_{h}\Diff(S^{1})_{hor}\cap \widetilde{V}$.  Further, these vector
fields are linearly independent.  Indeed, if we have $\{ a_{j} \}_{j=1}^{M}
\subset \R$ so that
\begin{align*}
\sum_{j=1}^{M}a_{j} G(\theta - \theta_{j}) = 0
\end{align*}
then for any $v$ we have
\begin{align*}
0 = \langle v, \sum_{j=1}^{M}a_{j} G(\theta - \theta_{j}) \rangle_{WP} = \sum_{j=1}^{M}a_{j}v(\theta_{j})
\end{align*}
and hence the only possible choice is that all $a_{j} = 0$.
\end{proof}
\end{proposition}
Now define the matrix
\begin{align*}
G_{ij} = \left\{ G(\theta_{i} - \theta_{j} ) \right\}
\end{align*}
Since 
\begin{align*}
 G(\theta_{i} - \theta_{j} ) = \left\langle  G(\cdot - \theta_{i} )  ,  G(\cdot - \theta_{j} ) \right\rangle_{WP}
\end{align*}
we see that this is the Gram matrix of a set of linearly independent vectors,
hence symmetric and positive definite.  We have the following formulas:
\begin{proposition}\label{prop:v-horizontal-lift}
The horizontal lift on $\widetilde{V}$ of the tangent vector $(v_{1}, ..., v_{M})
\in T_{\Theta}\lm$ is the vector field $\widetilde v(\theta)
\frac{\partial}{\partial \theta}$ for
\begin{align*}
\widetilde v(\theta) = \sum_{i=1}^{M}G(\theta - \theta_{i})u_{i} \frac{}{}\quad where \quad u_{i} = \sum_{j=1}^{M}G^{-1}_{ij}v_{j}
\end{align*}
Further,
\begin{align*}
\| \widetilde v \|_{WP}^{2} = \sum_{i,j}G^{-1}_{ij} v_{i}v_{j}
\end{align*}
\begin{proof}
The basis identified in Proposition \ref{prop:vector-field-basis} allows us to translate
this into a linear system, and the solution is as presented above.
%Clearly the vector field $\widetilde v$ above is horizontal.  We first verify
%that it does the right thing at the $\theta_{j}$'s:
%\begin{align*}
%\widetilde v(\theta_{k}) &= \sum_{i}G(\theta_{k} - \theta_{i})u_{i} \\
%&= \sum_{i}G_{ki}\sum_{j}G^{-1}_{ij}v_{j} \\
%&= \sum_{i,j} G_{ki}G^{ij}v_{j} \\
%&= \sum_{j} (GG^{-1})_{kj} v_{j} \\
%&= v_{k}
%\end{align*}
%We now compute the WP length:
%\begin{align*}
%\| \widetilde v \|_{WP}^{2} &= \left\langle \sum_{i}G(\cdot-  \theta_{i})u_{i}, \sum_{j}G(\cdot - \theta_{j})u_{j}\right\rangle_{WP} \\
%&= \sum_{i,j}G(\theta_{i} - \theta_{j}) u_{i}u_{j}  \\
%&= \sum_{i,j}G_{ji} \sum_{k}G^{-1}_{ik}v_{k} \sum_{l} G^{-1}_{jl}v_{l} \\
%&= \sum_{j,k,l} I_{jk} G^{-1}_{kl} v_{k} v_{l} \\
%&= \sum_{k,l} G^{-1}_{kl}v_{k}v_{l}
%\end{align*}
%Renaming the dummy variables completes the proof.
\end{proof}
\end{proposition}
We now seek to extend our result to all vector fields on $V$. We first make use
of the following simple fact:
\begin{lemma}\label{lemma:kernel-totality}
  For any configuration $\mathcal{L}^3$ of three distinct points on $S^1$, the
  subspace $\ker_V L = \mspan \{1, \sin, \cos\}$ is total for Dirac interpolation.
\end{lemma}
The important consequence of the above is that the coordinate map taking any
basis of $\ker_V L$ to Dirac evaluations on $\mathcal{L}^M$ can be represented
by an $M \times 3$ matrix of full rank.
\begin{lemma}\label{lemma:v-minimizer}
Let $G$ be an $M\times M$ positive matrix, $B$ an $M \times K$ full-rank matrix
with $K < M$. Then given some $w \in R^M$, the $G^{-1}$-orthogonal projection of
$w$ onto $\ker(B^T) = \ran (B)^\perp$ is given by 
\begin{align*}
  v = P_G^B w \doteq (I - G^{-1} B (B^T G^{-1} B)^{-1} B^T) w
\end{align*}
\end{lemma}
The proof of the above is an exercise in Lagrange multipliers. We are concerned
with the case when $G^{-1}$ is a Riemannian metric; however, in our case we only want
to use the metric for a subspace of $\R^M$ and is not intended for application
on all $\R^M$. Therefore, we seek to start on the subspace $\ran(B)^\perp$ and
extend the metric to all $\R^M$, assigning zero norm to any needed extensions.
In other words we wish to identify $P^L_G$ as the differential of a Riemannian
submersion.\aknote{Does this sentence make sense?}
\begin{lemma}
Assume that $G^{-1}$ is a metric on $\ker(B^T)$, where $B$ is a full-rank $M
\times K$ matrix with $K < M$. Then the norm-minimizing extension of $G^{-1}$ to
all $\R^M$ is given by  
\begin{align*}
  H = P_G^B G^{-1}.
\end{align*}
\end{lemma}
\begin{proof}
Given $\V{w}_1, \V{w}_2 \in \R^M$, apply the $G^{-1}$ metric to $P^B_G \V{w}_1$
and $P^B_G \V{w}_2$.
\end{proof}
By construction $H$ has rank $M-K$. This immediately yields the following.
\begin{corollary}
\label{corollary-green-gradient}
In the quotient space $\lm$, the gradient of the WP norm at $\Theta$ is
\begin{align*}
\frac{\partial}{\partial v_{j}} \| \widetilde v \|_{WP}^{2} = \left[ 2v^{T}H \right]_{j} 
\end{align*}
\begin{proof}
This is just the usual formula for the derivative of a quadratic form.
\end{proof}
\end{corollary}
Corollary \ref{corollary-green-gradient} is the first step to providing a
gradient for our optimization routine. 
%at each timestep yields a
%vector field on $[0,1] \times S^{1}$ which we can then project onto
%$T_{\phi}P_{h_{0}}$ to perform our optimization.

There is another way to see that the previous arguments yield the metric we
desire. If $v$ is a velocity field
corresponding to velocity field, then the momentum $L v$ is a sum of Dirac
delta functions. Since our manifold $\mathcal{L}^M$ is defined by a finite
number of point evaluations, this is equivalent to describing velocity fields by
momenta that are finite sums of Dirac delta functions. 

The question then is how does a momentum field described by an impluse train of
Dirac functions behave on this metric?  The Euler-Poincare differential equation
describes the flow of geodesics on Teichm\"{u}ller space. It is well-known that
self-similar solutions to this equation, known as {\em teichons}, exist. These
teichons can take the form of an impulse train. However, in order for the
Euler-Poincare equation to be well-posed, the coefficients of the impulse train
must satisfy certain constraints. Namely, the momentum field must be orthogonal
to $\ker_V L$ -- this is equivalent to asking for orthogonality to $\ran(B)$.
The natural metric on the momentum field is $G$, so we would like the
$G$-orthogonal projection onto $\ran(B)$. This turns out to be $P^B_G$.
Therefore, the metric on the $M$-dimensional space of momenta strengths on
$\mathcal{L}^M$ is given by $(P^G_B)^T G P^G_B = G P^G_B$, and on the $M$-dimensional space of
velocity strengths on $\mathcal{L}^M$, it is given by $P^B_G G^{-1}$.

Having computed the horizontal lifts satisfying the desired constraints, we will
find it useful to present an explicit formula.
\begin{corollary}\label{cor:v-field-wp-min}
Fix $\Theta$ and let the matrix $G$ be as in Proposition
\ref{prop:v-horizontal-lift}. For any $\V{v} \in T_\Theta \mathcal{L}^M$, 
\begin{align}\label{eq:v-discrete-minimizer}
  \| v \|^2_{\widetilde{W P}} = \min\{ (\V{v} - \V{w})^T G^{-1} (\V{v}-\V{w}) \}
\end{align}
where the minimization is performed over all $\V{w} \in \ran(B)$.
The horizontal lift $\widetilde{v}$ of $\V{v}$ to $V$ is given by
\begin{align*}
  \V{w} &= (B^T G^{-1} B)^{-1} B^T \V{v} \\
  \widetilde{v} &= \widetilde{w} + \sum_{j=1}^M \left( G^{-1} (\V{v}-G^{-1} B \V{w})
  \right)_j G(\cdot - \theta_j), \\
  \widetilde{w} &= \sum_{j=1}^3 \V{w}_j
  b_j(\cdot), \\
\end{align*}
where $\{b_j\}_{j=1}^3$ is the basis for $\ker_V L$ used to construct $B$:
$B_{m,k} = b_k(\theta_m)$. We will hereafter refer to $\V{m} = H\V{v}$ as the
momenta coefficients.
\end{corollary}

\noindent Thus for any $\V{v} \in T_\Theta \mathcal{L}^M$ we can identify a
corresponding element $\widetilde{v}$ from $T_h\mathbf{Diff}(S^1)_{hor}$; the
matrix $H = G^{-1} P^B_G$ also allows us to define an appropriate cotangent vector:
\begin{align*}
  v \mapsto L \widetilde{v} = \sum_{m=1}^M (H\V{v})_m \delta'_{\theta_m},
\end{align*}
where $\delta'_\theta$ is the Dirac measure $L^2$-orthogonalized against
$\ker_V L$ centered at $\theta \in S^1$.

\subsection{Other Subspaces}\label{sec:other-subspaces}
In the above section regarding computing the $W P$ norm on the Hilbert space
$V$, we chose Green's functions corresponding to the interpolating functionals
as the basis. While this produces the norm-minimal lift, we will see later a
reason to not use this basis for interpolation. If we want to choose a different
basis from which to interpolate, generalizing the results already obtained is
not difficult. 

In other words, this section is concerned with the resolution of the problem:
let $\widetilde{V}_N$ be any $N$-dimensional subspace of $\widetilde{V}$ that is
total for interpolation on $\delta(\mathcal{L}^M)$. For notational simplicity,
we let $\lambda$ denote the subspace 

Find $v \in \widetilde{V}_N$

Let $\lambda(\Phi)$ be the
corresponding map between coordinates on a basis of $\widetilde{V}_N$; i.e. if
$\phi_n(\cdot)$ are basis elements on $\widetilde{V}_N$, then the $M \times N$
matrix $\lambda(\Phi)$ has entries $\lambda(\Phi)_{m,n} = \langle \phi_n,
\delta_{\theta_m}\rangle_{W P} = \phi_n(\theta_m)$. Let $\Phi$ be the $N \times
N$ Gram matrix for the $\phi_n$: $\Phi_{m,n} = \langle \phi_m, \phi_n\rangle_{W
P}$. For $\V{v} \in \R^M$ interpolation data, define $\widetilde{V}_N(\V{v})$ as
the subset of functions from $\widetilde{V}_N \oplus \ker_V L$ that interpolate
to $\V{v}$. Then define
\begin{align*}
  \| \V{v} \|^2_{\widetilde{W P}, \widetilde{V}_N} = \min_{v \in \widetilde{V}_N (\V{v})} \| v\|^2_{W P}
\end{align*}
The results from the previous section may be rephrased by replacing $G \gets Q$
where $Q = \lambda(\Phi) \Phi^{-1} \lambda(\Phi)^T$:
\begin{align}\label{eq:other-subspace-norm}
  \| \V{v} \|_{\widetilde{W P}, \widetilde{V}_N}^2 &= \V{v}^T H \V{v} \\\nonumber
                &=: \V{v}^T \left(Q^{-1}  - Q^{-1} B ( B^T Q^{-1} B)^{-1} B^T
                Q^{-1}\right)\V{v} \\\nonumber
                &=: \V{v}^T Q^{-1} P^B_Q \V{v} \\\nonumber
                &=: \V{v}^T \V{m}.
\end{align}
However, unlike the result of Corollary \ref{cor:v-field-wp-min}, the momenta
coefficients $\V{m}$ here are not the reconstruction coefficients for the lift
unless $\widetilde{V}_N = \mathrm{span} \{ \delta_{\theta_m}, m = 1, \ldots, M\}$. The
coefficients are instead given by
\begin{subequations}
\label{eq:other-subspace-coefficients}
\begin{align}
  \V{w} &= \left(B^T Q^{-1}  B \right)^{-1} B^T Q^{-1} \V{v} \\
  \V{c} &= \Phi^{-1} \lambda(\Phi)^T Q^{-1} (\V{v} - B \V{w}).
\end{align}
\end{subequations}
From here, the reconstruction $\widetilde{v} \in \widetilde{V}_N \oplus \ker_V
L$ is given by 
\begin{align*}
  \widetilde{v} = \sum_{n=1}^N c_n \phi_n + \sum_{j=1}^3 w_j b_j
\end{align*}
It is not recommended to use \eqref{eq:other-subspace-norm} or
\eqref{eq:other-subspace-coefficients} to compute either the norm or any
coefficients. The matrices in the explicit formula given can easily be
ill-conditioned. We reformulate the problem in a format that allows for more
stable computation in Section \ref{sec:computations}.

\subsection{Computing path length}\label{sec:pathlength-notation}
The reason to $W P$ norms is to make computation of path lengths feasible. Again
we opt to instead use the energy \eqref{eq:energy-definition}. The velocity
field $v_s = \dot{\phi}_s \circ \phi_s^{-1}$ at discrete points in time will be
represented by discrete point-evaluations; we will assign the $W P$ norm using
the methodology of the previous section. 

%We now consider the following setup: let $f(s): S^1 \rightarrow S^1$ denote an
%$S^1$ diffeomorphism indexed by $s \in [0, 1]$. Suppose we are given $f(0)$ and
%$f(1)$. Our problem is then to find $f(s)$ such that $\int_0^1
%\|\left(\ppx{\theta} f(s)\right)^{-1} \ppx{s} f(s)\|^2_{A} \dx{s}$ is
%minimized. We assume that a unique minimum exists.  Let $v^s$ denote the velocity
%field $\left(\ppx{\theta} f(s)\right)^{-1} \ppx{s} f(s)$ at location $s$. We
%note that the velocity field is also given by $\ppx{s} f^{-1}(s)$.

%We let ${H}$ be $L^2_p$, the space of periodic $L^2$ functions on $[0,
%2\pi]$. The operator $\mathcal{L} = -{H} \left(\partial^3 +
%\partial\right)$
%(${H}$ is the periodic Hilbert transform) is semipositive and induces
%the Hilbert space ${A}$. The kernel of ${L}$ is the span of
%$\{1, \cos, \sin\}$. 

Our setup is a boundary-problem minimization: find $v_s$ subject to initial and
terminal conditions $\phi_0$ and $\phi_1$ such that $\int \|v_s
\|_{WP}^2 \dx{s}$ is minimized. We will adopt a Lagrangian approach
for this: we track $M$ particles on the domain of $\phi$ as they evolve in $s$.
(More formally, we choose $M$ values $\Phi_m$ on $S^1$ and track the particle locations
$q_m = \phi^{-1}_s(\Phi_m)$ along evolution in $s$.) To facilitate numerical simulation,
we divide $[0,1]$ into $T$ ordered subintervals $[0,1] = I^1 \cup I^2 \cup
\ldots I^T$ with stepsizes $|I^t| = h^t$ and $I^t = [s^{t,-}, s^{t,+}]$. Let
$\V{q}^t$ denote the $M$ particles at time $s^t = \frac{1}{2}\left(s^{t,-} +
s^{t,+}\right)$. Let $\V{v}^t$ denote $M$ velocity field evaluations at the same
time $s^t$, the midpoint of $I^t$. We assume that endpoint particle positions
$\V{q}^0$ (corresponding to $\phi^{-1}_0(\Phi)$) and $\V{q}^{T+1}$
(corresponding to $\phi^{-1}_1(\Phi)$) are given. We then use a symmetric
midpoint quadrature rule to integrate particle positions $\V{q}^t$:
\begin{align}\label{eq:explicit-particle-update}
  \V{q}^t &= \frac{1}{2}\left(\V{q}^0 + \sum_{r=1}^{t-1} h^r \V{v}^r +
  \frac{h^t}{2} \V{v}^t\right) + \frac{1}{2}\left( \V{q}^{T+1} - \sum_{r=t+1}^T
  h^r \V{v}^r - \frac{h^t}{2} \V{v}^t\right), & t\geq 1
  %\V{q}^t &= \frac{h^1}{2} \V{v}^1 + \sum_{r=2}^t h^r \V{q}^r, & r>1
\end{align}
Note that each element of $\V{q}^t$ then depends linearly on the velocity field
values $\V{v}^r$, $r \neq t$. In particular, collect all the velocity
evaluations into a matrix $V$, of size $M \times T$; do the same for the
particle positions in a matrix $Q$.  Then there exists a $T \times T$ matrix $Z$
such that 
\begin{align}\label{eq:particle-update}
  Q = \frac{1}{2} \left(Q^0 + Q^{T+1}\right) + V Z,
\end{align}
where $Q^0$ and $Q^{T+1}$ are matrices with the known vectors $\V{q}^0$ and
$\V{q}^{T+1}$ repeated. The matrix $Z$ has entries $Z_{r,t} = \frac{1}{2} c_{r,t} h_r$, where 
\begin{align}\label{eq:crt-def}
c_{r,t} = \left\{\begin{array}{rl} 
                   0, & r = t, \\
                   1, & r < t, \\
                   -1, & r > t.
                 \end{array}
          \right.
\end{align}
In order to evaluate the energy, which is $\int_0^1 \| v_s\|_{W P}^2 \dx{s}$, we
recall that the metric $\|\cdot\|_{\widetilde{WP},\widetilde{V}_N}$ determined
from the previous section has a factor of $h^t$ built into the norm, and
therefore 
\begin{align}\label{eq:pathlength-discretization}
  L = \sum_{t=1}^T \| \V{v}^t \|_{\widetilde{W P},\widetilde{V}_N}^2 = \sum_{t=1}^T 
  (\V{v}^t)^T Q^{-1} P_Q^B \V{v}^t = \sum_{t=1}^T (\V{v}^t)^T \V{m}^t,
\end{align}
where $Q^{-1}$ and $P_Q^B$ are time-varying, depending explicitly on $\V{q}^t$,
the particle locations at time $s^t$.


==> content/numerical-stein.tex <==
\section{Numerical Implementation}
We have described methods for computing the $WP$ norm of a velocity field and
the gradient of the energy for the minimization problem. These methods are
phrased in terms of integrals over an unbounded domain. Computing such integrals
with consistent accuracy is alone a challenging task. In an effort to simplify
the accuracy concerns, we seek to reduce the integration from an infinite
interval to a finite one. 

The informal argument is as follows: recall from Corollary
\ref{corollary-wp-norm} that the $WP$ norm of a velocity field $v$ is given by 
\begin{align*}
 \| v\|^2_{WP} = \int_0^{2\pi} \int_{-\infty}^\infty |v(\theta+s) + v(\theta-s) -
 2 v(\theta)|^2 \frac{1}{8\pi}\left(\frac{3}{s^4} - \frac{1}{s^2}\right) \dx{s}
 \dx{\theta}.
\end{align*}
Clearly the most important quantity to resolve in the integral is the
singularity of the kernel. Noting that the Laurent expansion of $\cot x$ is
$x^{-1} - x/3 + \ldots$, then we have
\begin{align*}
  \frac{1}{8\pi}\left(\frac{3}{s^4} - \frac{1}{s^2}\right) \sim \frac{3}{128\pi}
  \cot^4\left(\frac{s}{2}\right) + K,
\end{align*}
for some constant $K$ when $s$ is small. We might expect then that the above
relation allows us to compute Stein integrals by replacing the $1/s^\alpha$
kernel with a $\cot^\alpha(s/2)$ kernel and truncating the domain of integration
to one period in $s$. It turns out that truncation of the integral domain serves only
to augment the anticipated value of $K$ from the Laurent expansion.
\begin{theorem}\label{thm:wp-periodic-stein}
  For a smooth $v$, the $W P$ norm is given by 
  \begin{align*} 
    \|v \|^2_{W P} &= 
                  \frac{3}{128\pi} \int_0^{2\pi} \int_0^{2\pi} |v(\theta + s) + v(\theta - s)
  - 2 v(\theta)|^2 \left(\cot^4 \left(\frac{s}{2}\right) - 1\right)\dx{s}\dx{\theta}.
  \end{align*}
\end{theorem}
Our method of proof does not seem to offer any illumination into the result, so
we banish the details of proof to Appendix \ref{sec:periodic-stein}. It
is then not surprising that an analogue of Proposition
\ref{prop:gradient-length} giving an integral expression for the gradient of
path length can be proven with the same operations. We therefore present the
following without proof.
\begin{proposition}\label{prop:periodic-gradient-length}
The gradient of arclength for the fixed-endpoint problem satisfies
\eqref{eq:gradient-length}, with 
\begin{align}\label{eq:periodic-gradient}
 \nabla E (v)(t,\theta) = \frac{3}{128\pi} \int_0^{2\pi} \left(
 \cot^4\left(\frac{s}{2}\right) - 1\right) D_4 v(\theta,s)\dx{s},
\end{align}
where $D_4 v(\theta,s)$ is an unscaled approximation to the fourth derivative of
$v$ at $\theta$:
\begin{align*}
D_4 v(\theta,s) = v(\theta+2 s) - 4 v(\theta+ s)
   + 6 v(\theta) - 4 v(\theta-s) + v(\theta-2 s).
\end{align*}
\end{proposition}

\subsection{Discretization}
Let $K(s) = \frac{3}{64\pi} \left[ \cot^4(s/2) - 1\right]$. We need to compute
the two quantities
\begin{subequations}\label{eq:I-integral-goal}
\begin{align}\label{eq:I-integral-goal1}
  \| v \|^2_{WP} = \int_{0}^{2\pi} \int_0^\pi \left| D_2 v(\theta,s) \right|^2 K(s)
  \dx{s}\, \dx{\theta},
\end{align}
\begin{align}\label{eq:I-integral-goal2}
  \nabla E_v(\theta,t) =  \int_0^\pi D_4 v(\theta,s) K(s)
  \dx{s}.
\end{align}
\end{subequations}
The outer integral over $\theta$ is straightforward: assume that $[0,2\pi]$ is
covered by a non-overlapping collection of intervals $\Omega_k$ for $k = 1, 2,
\ldots, K$. Further, on each $\Omega_k$, let $\{\theta_n^k, w_n^k\}_{n=1}^N$ be
the $N$-point Gauss-Legendre quadrature rule. Then 
\begin{align*} 
  \int_0^{2\pi} f(\theta) \dx{\theta} \simeq \sum_{k=1}^K \sum_{n=1}^N w^k_n f(\theta^k_n),
\end{align*}
is an $h p$-adaptive discretization.  Define the inner integral
\begin{align*}
  I_\theta = \int_0^\pi f_\theta(s) K(s) \dx{s}.
\end{align*}
Let $\omega^{(\alpha,\beta)} = (1-r)^\alpha (1+r)^\beta$ be the Jacobi weight
function. Then change of variables yields
\begin{align*}
  I_\theta = \frac{3}{32\pi} \int_{-1}^1 f_\theta(s(r)) \frac{r}{(1-r)^2}
  \omega^{(-1/2, -1/2)} \dx{r},
\end{align*}
which is a Chebyshev approximation. We note that this is a straightforward
integral since for both cases \eqref{eq:I-integral-goal} the integrand
$f_\theta(s(r))$ is homogeneous of degree at least 2 at $s=0$ ($r=1$) so long as
$v_\theta$ is e.g. continuous and therefore the integrand of the Chebyshev
integral above is finite. We will use an $M$-point Chebyshev-Gauss-Radau
quadrature rule $\{r_m, u_m\}$ to approximate the integral; the fixed quadrature node will lie
at $r=-1$.

Now the full discretizations of \eqref{eq:I-integral-goal} are given by
\begin{subequations}\label{eq:I-discretization}
\begin{align}\label{eq:I-discretization-length}
  \|v \|_{W P}^2 \simeq \frac{3}{32 \pi} \sum_{k=1}^K \sum_{n=1}^N w^k_n
  \sum_{m=1}^M \frac{u_m r_m}{(1-r_m)^2} D_2^2 v(\theta^k_n, s(r_m)),
\end{align}
\begin{align}\label{eq:I-discretization-gradient}
  \nabla E(v)(\theta^k_n) \simeq \frac{3}{32 \pi} \sum_{m=1}^M
  \frac{u_m r_m}{(1-r_m)^2} D_4 v(\theta^k_n, s(r_m)),
\end{align}
\end{subequations}
where $s(r) = \arccos r$. Note that the difficulty with the above formulas is
the need to evaluate the velocity field at various locations $\theta^k_n \pm
\arccos(r_m)$. Although the $\arccos(r_m)$ are equidistant, the lack of symmetry
in $\theta^k_n$ requires us to evaluate $v$ at unpredictable locations. For now,
we use linear interpolation of known samples $v(\theta^k_n)$.

\begin{comment}
  Let $K(s) = \frac{3}{64\pi} \cot^4\left(\frac{s}{2}\right)$ and $D_2 v(\theta,s)
  = v(\theta+s) + v(\theta-s) - 2v(\theta)$. Then Theorem
  \ref{thm:wp-periodic-stein} states
  \begin{align*}
    \|v \|^2_{W P} &= \frac{1}{2} \int_0^{2\pi} \int_0^{2\pi} \left|
    D_2v(\theta,s)\right|^2 K(s) \dx{s}\dx{\theta} - 
                     \frac{3}{128\pi} \int_0^{2\pi} \int_0^{2\pi} \left|
           D_2v(\theta,s)\right|^2 \dx{s}\dx{\theta} \\
    &= \int_0^{2\pi} \int_0^\pi \left|D_2v(\theta,s)
        \right|^2 K(s) \dx{s} \dx{\theta} - \frac{9}{32} \|v \|^2.
  \end{align*}
  The non-singular term $\|v \|^2$ is not the difficult portion to calculate. We
  will eventually be concerned with non-equidistant grids. Therefore, assume that
  $[0,2\pi]$ is covered by a non-overlapping collection of intervals $\Omega_k$
  for $k = 1, 2, \ldots, K$. Further, on each $\Omega_k$, let $\{\theta_n^k,
  w_n^k\}_{n=1}^N$ be the $N$-point Gauss-Legendre quadrature rule. Then 
  \begin{align*}
    \| v \|^2 \simeq \sum_{k=1}^K \sum_{n=1}^N w^k_n v^2\left(\theta^k_n\right),
  \end{align*}
  is an $h p$-adaptive discretization for $\|v \|^2$ (state convergence). The more
  difficult quantity to evaluate is the inner integral
  \begin{align*}
    \int_0^\pi |w_\theta(s)|^2 K(s) \dx{s},
  \end{align*}
  where $w_\theta(s) := D_2 v(\theta,s)$. The integral is
  singular and so we must adopt unconventional quadrature methods. Using the
  change of variable $r \gets \cos s$, then the above integral reduces to 
  \begin{align*}
   I_\theta = \frac{3}{64\pi}\int_{-1}^1 w_\theta(s(r)) \wjacobi{-\frac{5}{2}}{\frac{3}{2}} \dx{r},
  \end{align*}
  where $\omega^{(\alpha,\beta)} = (1-r)^\alpha (1+r)^\beta$ is the Jacobi weight
  function. Now if we expand $w_\theta(s(r))$ in a sequence of generalized Jacobi
  polynomials (cite), we obtain
  \begin{align*}
    w_\theta(s(r)) = \sum_{n=0}^\infty \hat{w}_n p_n^{(-\frac{5}{2},
    \frac{3}{2})}.
  \end{align*}
  Our definition of generalized Jacobi polynomial differs from established
  practice:
  \begin{align*}
   p_n^{(-\frac{5}{2}, \frac{3}{2})} = (1-r) p_n^{(-1/2,3/2)}.
  \end{align*}
  With this, then 
  \begin{align*}
    I_\theta = \frac{3}{64\pi} \sum_{n} |\hat{w}_n|^2.
  \end{align*}
  For the discretization, we need to choose the points $\{s_n\}_{n=1}^N$ that
  allow us to approximate $\hat{w}$. Note that since $w_\theta(s)$ as $s \downarrow
  0$ is a second difference operator, then as long as $v(\theta)$ is
  differentiable at that point, then $w_\theta(s)$ is homogeneous of at least
  degree 1 at the origin ($s=0$) and therefore $w_\theta(s(r)) \times (1-r)^{-1}$ is not
  singular at $r=1$. Therefore, defining $q = w_\theta \times (1-r)^{-1}$ then we
  seek an $L^2_{(-1/2, 3/2)}$ expansion
  \begin{align*}
    q = \sum_{n=0}^\infty \hat{q}_n p_n^{(-1/2, 3/2)}.
  \end{align*}
  At this stage there are several possible choices for discretization points. For
  example, if we choose the $(-\frac{1}{2}, \frac{3}{2})$ Jacobi-Gauss points,
  which we label as $\{r_m, u_m\}_{m=1}^M$, then 
  \begin{align*}
    I_\theta \simeq \frac{3}{64\pi}\sum_{m=1}^M \frac{u_m}{(1-r_m)^2} w^2_\theta(s(r_m)).
  \end{align*}
  We have now obtained a discretization for \eqref{eq:periodic-gradient}: 
  \begin{align}\label{eq:periodic-gradient-discretization}
   \nabla E(v)(\theta, t) \simeq \frac{3}{64\pi} \sum_{m=1}^M
   \frac{u_m}{(1-r_m)^2} D_4 v(\theta, s(r_m)) - 
  \end{align}
  the above
  equation with $w^2_\theta(s(r_m))$ replaced by the evaluations $D_4 v(\theta,
  s(r_m))$.
  To complete computation of the $WP$ norm, all that remains is to integrate
  $I_\theta$ over $\theta$ for which we employ a method identical to that
  described for $\| v\|^2$.  When all is finished, we obtain
  \begin{align*}
    \| v \|_{W P}^2 \simeq \frac{3}{32} \sum_{k=1}^K \sum_{n=1}^N w^k_n \left[ -3 v^2(\theta^k_n)
       + \frac{1}{2\pi}\sum_{m=1}^M \frac{u_m}{(1-r_m)^2} \left( v(\theta^k_n + \acos r_m) +
               v(\theta^k_n - \acos r_m) - 2 v(\theta^k_n)\right)^2 \right].
  \end{align*}
  With an absence of exploitable symmetry, the above expression requires a total
  of $M N K$ evaluations of $v$, which can be prohibitively expensive.
\end{comment}

\subsection{Temporal discretization}
We discretize time into an increasing sequence $\{t_0, t_1, \ldots, t_T\}
\subset [0, 1)$, with $t_0 = 0$ (it is unnecessary to consider the velocity
field at $t=1$). If the Lagrangian velocity $v_j(t)$ is a smooth function, (is
it?) then it makes sense to use a high-order discretization of the temporal
interval, rather than e.g. a first-order equidistant method. For example,
consider the $(T+1)$-point Legendre-Gauss-Radau quadrature rule $\{t_q, w_q\}$
over $[0,1)$ with fixed node at $t=0$. Then the constraint from
\eqref{eq:velocity-constraints} becomes $F_j(v) = \sum_{q=0}^{T} v_j(t_q) w_q$,
and now $D F$ may be computed in a straightforward manner, along with the
necessary dimension-$T$ kernel for the projection in Lemma
\ref{lemma:v-projection}. Note that an easy way to implement the projection onto
the kernel of $D F$ is given by the matrix $I - \kappa \mathbf{w} \mathbf{w}^T$,
where $\mathbf{w}$ is a vector with entries $w_q$ and $\kappa =
1/\|\mathbf{w}\|^2_2$.  The temporal discretization also allows us to compute the
path length:
\begin{align}\label{eq:T-discretization}
 E = \sum_{q=0}^T w_q \| v(t_q) \|_{WP}.
\end{align}
Note that to compute intermediate shapes at times $t_q$ for $q>0$, a simple
truncation of the quadrature rule is not accurate. Instead, use of this
high-order quadrature rule implicitly endows the temporal samples of
$v_j(t)$ with a degree-$T$ interpolatory polynomial. The intermediate welding
maps $\phi_{t_q}$ are then given by computing the primitive of this polynomial
and evaluating it at the appropriate temporal locations:
\begin{align}\label{eq:phi-interpolation}
  \phi_{t_i}(\theta) = \phi_0(\theta) + \sum_{q=0}^T w_{i,q} v(t_q, \theta),
\end{align}
where $w_q \equiv w_{T,q}$. At $t=1$ this procedure is a more complicated, but
equivalent way of implementing the quadrature rule. 

\subsection{The minimization algorithm}
All of the above described elements are put together in a minimization algorithm
that we use to find the geodesic in $\Homeo(S^1)$ connecting a shape to a
circle. The steps are outlined in Listing \ref{alg:minimization}.
\begin{algorithm}
  \caption{The miminization algorithm for computing geodesics between shapes.}
  \label{alg:minimization}
  \input{algorithms/minimization}
\end{algorithm}
In addition to projecting out elements in the rowspan of $D F$ we also project
out any part of $\nabla E$ that recharts the intermediate welding maps.
Throughout the computation the `interior' discretization of $S^1$ given by
$\theta_{-,n}^k$ remains constant and the pairs $\{(\theta_{-,n}^k,
\theta_{+,n}^k(t_q))\}$ represent domain-image pairs of the map $\phi_{t_q}$. A
geodesic flow at equidistant times is depicted in Figure
\ref{fig:camel-geodesic}.
\begin{figure}
  \begin{center}
    \includegraphics[width=6in]{images/camel-geodesic/camel.pdf}
  \end{center}
  \caption{Geodesic flow of a camel shape to the identity map (a circle). The
  computed $W P$ distance is 16.3252. The snapshots are equidistant in time, and
  evolve from top to bottom, then from left to right.}
  \label{fig:camel-geodesic}
\end{figure}

Here are things I haven't yet gotten to work:
\begin{itemize}
\item Multiple charts -- this is a big deal since there are lots of shapes I
      can't even start minimization on without this. The difficulty I'm having
      right now with this is the gluing together of the charts -- it's more
      intensive than I first thought.
\item The $N$, $K$ discretization described above yet isn't quite done yet...the
      reason is that there's a regularity concern that I have to flesh out and deal
      with. Until I do that, I'm just using a cubic interpolation procedure with $N=2$.
\end{itemize}
Some observations based on my simulations:
\begin{itemize}
  \item I'm not convinced that I'm able to compute the minimum. Here are things
  that seem to look good:
  \begin{itemize}
    \item I only `go downhill', so every iteration does decrease the path length
    \item The norm of the gradient (numerical matrix norm -- means nothing
    physically) decreases as well
    \item The process seems to slow to a minimum, i.e. the decrease in path
    length at each iteration decreases, and I'm forced to take smaller and
    smaller steps in the direction of the gradient.
  \end{itemize}
  And here are things that look bad:
  \begin{itemize}
    \item Firstly, you should take a look at the camel and see if it makes
      sense. I feel like the kinks aren't smoothed out quickly enough, but I don't
      know.
    \item The norm of the gradient is still super-large at the end of the
    iteration, ~1e5. (Though it decreases from a much higher value.)
  \end{itemize}
  \item There are lots of discretization parameters to play around with; here's
  my take on things:
  \begin{itemize}
    \item The temporal discretization, $T$, seems ok. The limited tests I've
    done are pretty insensitive to the value of $T$ when it's greater than 20 or
    so.
    \item $s$-discretization $M$ -- this is a question mark. I'm using 200
    points right now, which seems fine, and making it larger doesn't seem to do
    much more. I'm actually fairly confident that it's accurate. And for
    reference, I've tested equations \eqref{eq:I-discretization} on cosine
    functions for wavenumbers up to about 20 and it gives what one expects.
    \item $\theta$-discretization $N$, $K$. I think this is the bottleneck.
    Right now my initial choice of points is just to do (a) equidistant on
    $\theta_-$; (b) equidistant $\theta_+$; (c) the input/output pairs from
    zipper; and then I union them all. The converged WP norm value does depend
    non-trivially on the number of points, and this is a sign either that (1)
    something's not right, or (2) more likely that enough points just haven't
    been used yet.
  \end{itemize}
  \item I'm randomly fixing the chart by imposing $\phi_t(\theta_j) = \theta_j$
  for $j=1,2,3$. I take $\theta_j$ equispaced. This is enforced by adding these
  points to the discretization list and then forcing the velocity to zero, which
  is equivalent to a projection. I guess this isn't mathematically necessary,
  but it does make me feel better :)
\end{itemize}
And here are things that I'm trying to get moving:
\begin{itemize}
  \item Multiple charts -- obviously. If I can get this to work then I think
  there isn't a shape I can't compute. Now whether the computation is correct is
  a different matter entirely.
  \item I want to start with some intermediate shapes computed from a shape, and
  compute the geodesic from those intermediate shapes to the identity. Obviously
  I should get the same thing, and this would be a good way to check the math.
  \item If I understand correctly, you posit that mapping shape $A$ to $B$ just
  requires mapping each to the circle and then daisy-chaining the geodesics to
  ge the full geodesic, right? Well, I can go ahead and try this.
\end{itemize}


==> content/old-gradient-section.tex <==
\subsubsection{Green's function and the gradient of arclength}

This material appears for the case of $\R^{n}$ in [CITE Mumford]; we repeat it here in the case of $S^{1}$ in order to be self-contained.  Let $\mathcal{L}^{M}$ be the space of configurations of $M$ points $\theta_{1} < \theta_{2} < ... < \theta_{M}$ on the unit circle and write $\Theta = \left\{ \theta_{1}, \theta_{2}, ..., \theta_{M}  \right\}$. The tangent space $T_{\Theta}\lm$ is the $M$-dimensional space of vector fields $v = (v_{1}, v_{2}, ..., v_{M})$ supported on the set $\Theta$.  We consider all possible extensions of $v$ to vector fields defined on the entire circle, and induce a metric on $\lm$ by defining the norm
\begin{align}\label{eq:v-global-minimizer}
\| v \|_{\widetilde{WP}} \equiv \inf \left\{ \| \widetilde v \|_{WP} : \widetilde{v}(\theta_{j}) = v_{j}  \right\}
\end{align}
Having chosen some basepoint $\Theta$, the tangent space $T_{h}\Diff(S^{1})$ then splits as the direct sum
\begin{align*}
T_{h}\Diff(S^{1}) = T_{h}\Diff(S^{1})_{hor} \oplus T_{h}\Diff(S^{1})_{ver}
\end{align*}
The vertical subspace is the subspace consisting of vector fields which vanish at all the $\theta_{j}$.  The horizontal subspace is the $M$-dimensional orthogonal complement of the vertical subspace and hence contains the norm-minimizing extensions of vectors in $T_{\Theta}\lm$, known as the \textit{horizontal lifts}.
\aknote{I have some concerns about this statement: I don't doubt it's true, but
I think we have to talk about what $v(\theta)$ means -- is it true Dirac
evaluation in the extended $L^2$ sense? Or is it Dirac evaluation in the operator
$\mathcal{L}$ sense? If it's the former (which is what we're computing), then I
don't think the following proposition is correct.}

Working in coordinate $v$ on $P_{h_{0}}$, we may obtain an expression for the
gradient of arc length by considering Green's function for the WP differential
operator $L = -\mathcal{H}(\partial^{3} - \partial)$ ($\mathcal{H}$ is the Hilbert
transform).  This Green's function is known explicitly, see
\cite{kushnarev_teichons_2009}:

\begin{align*}
G(\theta) = 2 \sum_{n=2}^{\infty} \frac{\cos(n\theta)}{(n^{3}-n)} = (1-\cos \theta) \log\left[ 2(1-\cos \theta)  \right] + \frac{3}{2}\cos \theta -1
\end{align*}

\begin{proposition}
The set of vector fields
\begin{align*}
\left\{ G(\theta, \theta_{j}) \frac{\partial}{\partial\theta} \right\}_{j=1}^{M}
\end{align*}
is a basis for the horizontal subspace $T_{h}\Diff(S^{1})_{hor}$
\begin{proof}
By the reproducing kernel property of Green's function, we know that 
\begin{align*}
\langle v, G(\cdot - \theta_{j}) \rangle_{WP} = v(\theta_{j})
\end{align*}
for all $j = 1,2,...,M$ and any vector $v \in T_{h}\Diff(S^{1})$.  In particular, if $v$ is vertical we have
\begin{align*}
\langle v, G(\cdot - \theta_{j} )\rangle_{WP} = v(\theta_{j}) = 0
\end{align*}
so $G\frac{\partial}{\partial\theta}$ is orthogonal to the vertical subspace; i.e. $v \in T_{h}\Diff(S^{1})_{hor}$.  Further, these vector fields are linearly independent.  Indeed, if we have $\{ a_{j} \}_{j=1}^{M} \subset \R$ so that
\begin{align*}
\sum_{j=1}^{M}a_{j} G(\theta - \theta_{j}) = 0
\end{align*}
then for any $v$ we have
\begin{align*}
0 = \langle v, \sum_{j=1}^{M}a_{j} G(\theta - \theta_{j}) \rangle_{WP} = \sum_{j=1}^{M}a_{j}v(\theta_{j})
\end{align*}
and hence the only possible choice is that all $a_{j} = 0$.
\end{proof}
\end{proposition}
Now define the matrix
\begin{align*}
G_{ij} = \left\{ G(\theta_{i} - \theta_{j} ) \right\}
\end{align*}
Since 
\begin{align*}
 G(\theta_{i} - \theta_{j} ) = \left\langle  G(\cdot - \theta_{i} )  ,  G(\cdot - \theta_{j} ) \right\rangle_{WP}
\end{align*}
we see that this is the Gram matrix of a set of linearly independent vectors, hence symmetric and positive definite.  We have the following formulas:
\begin{proposition}\label{prop:v-horizontal-lift}
The horizontal lift of the tangent vector $(v_{1}, ..., v_{M}) \in T_{\Theta}\lm$ is the vector field $\widetilde v(\theta) \frac{\partial}{\partial \theta}$ for
\begin{align*}
\widetilde v(\theta) = \sum_{i=1}^{M}G(\theta - \theta_{i})u_{i} \frac{}{}\quad where \quad u_{i} = \sum_{j=1}^{M}G^{-1}_{ij}v_{j}
\end{align*}
Further,
\begin{align*}
\| \widetilde v \|_{WP}^{2} = \sum_{i,j}G^{-1}_{ij} v_{i}v_{j}
\end{align*}
\begin{proof}
Clearly the vector field $\widetilde v$ above is horizontal.  We first verify that it does the right thing at the $\theta_{j}$'s:
\begin{align*}
\widetilde v(\theta_{k}) &= \sum_{i}G(\theta_{k} - \theta_{i})u_{i} \\
&= \sum_{i}G_{ki}\sum_{j}G^{-1}_{ij}v_{j} \\
&= \sum_{i,j} G_{ki}G^{ij}v_{j} \\
&= \sum_{j} (GG^{-1})_{kj} v_{j} \\
&= v_{k}
\end{align*}
We now compute the WP length:
\begin{align*}
\| \widetilde v \|_{WP}^{2} &= \left\langle \sum_{i}G(\cdot-  \theta_{i})u_{i}, \sum_{j}G(\cdot - \theta_{j})u_{j}\right\rangle_{WP} \\
&= \sum_{i,j}G(\theta_{i} - \theta_{j}) u_{i}u_{j}  \\
&= \sum_{i,j}G_{ji} \sum_{k}G^{-1}_{ik}v_{k} \sum_{l} G^{-1}_{jl}v_{l} \\
&= \sum_{j,k,l} I_{jk} G^{-1}_{kl} v_{k} v_{l} \\
&= \sum_{k,l} G^{-1}_{kl}v_{k}v_{l}
\end{align*}
Renaming the dummy variables completes the proof.
\end{proof}
\end{proposition}
This immediately yields the following.
\begin{corollary}
\label{corollary-green-gradient}
In the quotient space $\lm$, the gradient of the WP norm at $\Theta$ is
\begin{align*}
\frac{\partial}{\partial v_{j}} \| \widetilde v \|_{WP}^{2} = \left[ 2v^{T}G^{-1} \right]_{j} 
\end{align*}
\begin{proof}
This is just the usual formula for the derivative of a quadratic form.
\end{proof}
\end{corollary}
Applying corollary \ref{corollary-green-gradient} at each timestep yields a vector field on $[0,1] \times S^{1}$ which we can then project onto $T_{\phi}P_{h_{0}}$ to perform our optimization.


==> content/pathvariation.tex <==
\newpage
Let $q = q(t,x,s)$ with $q_j$ the partial derivative of $q$ with respect to the $j$th argument. For brevity we also write $q(t,x,s) = q$. A functional inverse is denoted $q^{-1}$ whereas a multiplicative inverse is surrounded by parens: $(q)^{-1}$. Compositions $\circ$ are with respect to the second argument. So e.g. $v(t,x,s) = \left(\ppx{t} q(t, x,s)\right)|_{x=q^{-1}(x,t,s)} = q_1 \circ q^{-1}$. On $\mathcal{P}$ we have the defined norm 
$\left\| v_3 \right\|_{W P}$. 
%Since discrete approximation of the norm $\| \cdot \|_{W P}$ can be accomplished in a quadratic form with the operator $L_F$, 
We now expres this norm in terms of $q_{1,3} \circ q^{-1}$, which is the unconstrained gradient.
We first note that 
\begin{subequations}\label{eq:misc-props}
\begin{align*}
  0 = \ppx{s} q \circ q^{-1} &= \ppx{s} q(t, q^{-1}(t,x,s), s) \\
  &= \ppx{s} q_2(t, q^{-1}(t,x,s), s) \ppx{s} q^{-1}(t,x,s) + q_3(t, q^{-1}(t,x,s), s)
\end{align*}
so that
\begin{align}\label{eq:misc-propsa}\nonumber
  \ppx{s} q^{-1}(t,x,s) &= -q_3(t,q^{-1}(t,x,s),s) \left[ q_2 (t, q^{-1}(t,x,s), s)\right]^{-1}.\\
                        &= -\left(q_3 \circ q^{-1}\right) \left(q_2 \circ q^{-1}\right)^{-1}
\end{align}
Also, we have $x \equiv q \circ q^{-1}$ so that
\begin{align}\label{eq:misc-propsb}
  1 = \ppx{x} q \circ q^{-1} %\\\nonumber
    = \ppx{x} q(t, q^{-1}(t,x,s), s) %\\
    = \left(q_2 \circ q^{-1}\right) \ppx{x} q^{-1}.
\end{align}
Finally we derive an expression for $\ppx{x} v$:
\begin{align}\label{eq:misc-propsc}%\nonumber
  v_2 = \ppx{x} v &= \ppx{x} (q_1 \circ q^{-1}) %\\\nonumber
            = \ppx{x} q_1(t, q^{-1}, s) %\\
            = \left(q_{1,2} \circ q^{-1}\right) \ppx{x} q^{-1}
\end{align}
\end{subequations}
Putting all these together we have
\begin{align*}
   v_3 =\ppx{s} v &= \ppx{s} q_1(t, q^{-1}(t,x,s), s) \\
             &= q_{1,2}(t, q^{-1}(t,x,s), s) \ppx{s} q^{-1}(t,x,s) + 
             q_{1,3} (t, q^{-1}, s) \\
             &\stackrel{\eqref{eq:misc-propsa}}{=}  -\left(q_{1,2} \circ q^{-1}\right) \left(q_3\circ q^{-1}\right) \left( q_2 \circ q^{-1}\right)^{-1} + q_{1,3} \circ q^{-1} \\
             &\stackrel{\eqref{eq:misc-propsc}}{=} -v_2 \left(\ppx{x} q^{-1}\right)^{-1} \left(q_3\circ q^{-1}\right) \left( q_2 \circ q^{-1}\right)^{-1} + q_{1,3} \circ q^{-1} \\
             &= -v_2 \left(q_3 \circ q^{-1}\right) \left[\left(\ppx{x} q^{-1}\right) (q_2 \circ q^{-1})\right]^{-1} + q_{1,3} \circ q^{-1} \\
             &\stackrel{\eqref{eq:misc-propsb}}{=} -v_2 (q_3 \circ q^{-1}) + q_{1,3} \circ q^{-1} \\
             &= -v_2 \left(\int_0^\xi q_{1,3}(\xi,q^{-1},s) \dx{\xi}\right) + q_{1,3} \circ q^{-1} \\
             %&= -v_2 \left(\int_0^t (q_{1,3} \circ q^{-1})|_{t=\xi} \dx{\xi}\right) + q_{1,3} \circ q^{-1} \\
             &= \left[ \mathrm{Id} - v_2 \int_0^t (\cdot) \dx{\xi}\right] \left(q_{1,3} \circ q^{-1}\right)
\end{align*}

We have thus shown that
\begin{align*}
  \pfpx{\left(\dot{q} \circ q^{-1}\right)_{t;r}}{r}(x) &= \mathcal{Y}\left[ \pfpx{v}{s}\right],
\end{align*}
where the linear operator $\mathcal{Y}$ is given by 
\begin{align}\label{eq:operator-Y-definition2}
  \mathcal{Y}(t,x,s) = \mathrm{Id} - v' \int_0^t (\cdot)_{\xi} \dx{\xi}
\end{align}


==> content/stein-extension.tex <==
For any $\alpha>0$, let $H^\alpha$ be the $L^2$ Sobolev space. 
%and define the seminorm
%\begin{align*}
% \left| f \right|_{H^\alpha}^2 = \sum_{k\in\Z} (k^2)^\alpha
% \left|\hat{f}_k\right|^2.
%\end{align*}
Also, let $\Delta_{A}[f](\theta; s)$ be any 
finite-difference approximation to the order $A\in\N$ derivative of $f$ using an
equidistant mesh of size $s$ at the location $\theta$. For example we could
define $\Delta_2$ as the symmetric second-difference operator: $s^2 \Delta_2[f](\theta;s) =
f(\theta+s) + f(\theta-s) - 2 f(\theta)$.
\begin{theorem}
  Let $f : S^1 \rightarrow \R$ be an $H^\alpha$ function, and denote $A =
  \lceil \alpha \rceil$. Then
  \begin{align*}
    \left\| f^{(\alpha)} \right\|^2
    = b(\alpha, \Delta_A)\left\| \int_0^\infty 
        \frac{\Delta_A[f](\theta;s)}{s^{\alpha - A + \frac{1}{2}}} \dx{s} \right\|^2
    %\int_0^{2\pi} \int_0^\infty 
    %  \frac{\left|\Delta_{A}[f](\theta; s)\right|^2}
    %       {s^{1 + 2\alpha}} 
    %  \dx{s}\,\dx{\theta},
  \end{align*}
  where the constant $b$ is given by 
  \begin{align*}
    b(\alpha, \Delta_A) = \int_0^\infty \frac{\left| \Delta_A[e^{i x}](0; s)\right|^2}{s^{2
    \alpha-2 A+1}} \dx{s}.
  \end{align*}
\end{theorem}


==> content/wp-metric.tex <==
Given a simply-connected planar region $\Omega$ bounded by a smooth Jordan curve (this is our definition of a ``shape''), one may construct a pair of conformal maps $\Phi_{+}: \Delta_{+} \to \Omega_{+}$ and $\Phi_{-}: \Delta_{-} \to \Omega_{-}$, which map the interior and exterior of the unit disk to the interior and exterior of $\Omega$, respectively.  These maps extend continuously to the boundary $S^{1}$, and their composition $\Phi_{+}^{-1} \circ \Phi_{-}$, restricted to the boundary, is a map $\Psi: S^{1} \to S^{1}$.  This construction is almost an isomorphism: the space of shapes, modulo translation and scale, is isomorphic to the group $\Diff(S^{1})$, modulo conformal self-maps of the disk.  This provides an elegant way of making the space of shapes into a metric space;  we take an equivalence class of diffeomorphisms of the circle as a representation of a shape.  In the mathematical literature, these homeomorphisms of $S^{1}$ are commonly known as ``welding maps''.

Let $v$ be a vector field on $\Chat$ which is holomorphic on $\Omega^{*}$ and vanishes at infinity.  Then the WP norm of $v$ at the point $\partial \Omega$ is defined as follows.
\begin{definition}[Weil-Peterson norm]
\begin{align*}
\| v \|_{WP}^{2} \equiv \iint_{\Omega} \left| \bar \partial v
\right|^{2}\rho_{\Omega}^{2} d^{2}u
\end{align*}
where $\rho_{\Omega}^{2}d^{2}u$ is hyperbolic area on $\Omega$.
\end{definition}
\noindent However, we wish to work in terms of welding maps, rather than working directly on shapes.  This reduces a problem in 2 dimensions to a problem about functions on the circle.  Applying results of Ahlfors and Beurling, one may work out the corresponding norm on the tangent spaces to $\Diff(S^{1})$.  If $w(\theta) = \sum_{n=-\infty}^{\infty} a_{n} e^{in\theta} \frac{\partial}{\partial \theta}$ is a vector field on the circle, one finds that
\begin{align}\label{eq:wp-norm-fourier}
\| w \|_{WP}^{2} = \sum_{n=2}^{\infty} (n^{3}-n) |a_{n}|^{2} = \frac{\left\|
w^{(3/2)} \right\|^2 - \left\|w^{(1/2)}\right\|^2}{2},
\end{align}
where $\left\|\cdot\right\|$ denotes the $L^2$ norm. This formula, while explicit, is troublesome in numerical computations; the boundary values of conformal maps have so much high-frequency content, even for curves with real-analytic boundaries, that the number of Fourier coefficients required for for an accurate global representation is prohibitive. 


==> pgf-external.tex <==
\long\def\beginpgfgraphicnamed#1#2\endpgfgraphicnamed{\includegraphics{#1}}

